HOP, UNION, GENERATE: Explainable Multi-hop Reasoning without Rationale Supervision

Explainable multi-hop question answering (QA) not only predicts answers but also identifies rationales, i. e. subsets of input sentences used to derive the answers. This problem has been extensively studied under the supervised setting, where both answer and rationale annotations are given. Because rationale annotations are expensive to collect and not always available, recent efforts have been devoted to developing methods that do not rely on supervision for rationales. However, such methods have limited capacities in modeling interactions between sentences, let alone reasoning across multiple documents. This work proposes a principled, probabilistic approach for training explainable multi-hop QA systems without rationale supervision. Our approach performs multi-hop reasoning by explicitly modeling rationales as sets, enabling the model to capture interactions between documents and sentences within a document. Experimental results show that our approach is more accurate at selecting rationales than the previous methods, while maintaining similar accuracy in predicting answers.

==> exNLP_acl2023 (Copy)/abstract.tex <==
\begin{abstract}
    %Multi-hop question answering (QA) often involves two parts -- identifying relevant information and predicting an answer.
    %Multi-hop question answering (QA) predicts both answers and sentence-level rationales.
    %To deploy reading comprehension systems in the real world, it is important to understand how their decisions are made.
    % Multi-hop reasoning plays an important role in reading comprehension.
    % To evaluate a question answering (QA) system's ability to perform multi-hop reasoning, 
    % Multi-hop QA has been extensively studied in the supervised setting, where both rationale and answer annotations are given.
    % Because annotating sentence-level rationales is expensive, recent efforts have thus been devoted to developing unsupervised methods.
    % However, existing unsupervised methods can only reason about different pieces of information with very limited capacities.
    % This work proposes a principled, probabilistic approach for multi-hop QA. 
    Explainable multi-hop question answering (QA) not only predicts answers but also identifies rationales, i. e. subsets of input sentences used to derive the answers.
    %Existing methods rely on supervision for both answers and rationales.
    This problem has been extensively studied under the supervised setting, where both answer and rationale annotations are given.
    Because rationale annotations are expensive to collect and not always available, recent efforts have been devoted to developing methods that do not rely on supervision for rationales.
    However, such methods have limited capacities in modeling interactions between sentences, let alone reasoning across multiple documents.
    This work proposes a principled, probabilistic approach for training explainable multi-hop QA systems without rationale supervision.
    Our approach performs multi-hop reasoning by explicitly modeling rationales as sets,
    enabling the model to capture interactions between documents and sentences within a document.
    Experimental results show that our approach is more accurate at selecting rationales than the previous methods, while maintaining similar accuracy in predicting answers.
\end{abstract}

==> exNLP_acl2023 (Copy)/analysis.tex <==
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/plot.pdf}
%     \caption{Comparison between parallel reasoning and sequential reasoning on the number of examples that are predicted correctly and on the ratio of how many correct predictions are made with the right reasons. Results are on the HotpotQA test set.}
%     \label{fig:sequential_parallel_results}
% \end{figure}
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
%  & Ans EM & Doc Acc & Partial Doc Acc \\ \midrule
% Ind. & 55.7 & 49.3 & 97.4 \\
% Joint & \textbf{60.0} & \textbf{76.9} & \textbf{99.1} \\
% \bottomrule
% \end{tabular}
% \begin{tabular}{lccc}
% \toprule
%  & Ans EM & Doc Acc & Partial Doc Acc \\ \midrule
% Ind. & 55.7 & 49.3 & 97.4 \\
% Joint & \textbf{60.0} & \textbf{76.9} & \textbf{99.1} \\
% \bottomrule
% \end{tabular}
% \begin{tabular}{lcc}
% \toprule
%  & Ans EM & Doc EM \\ \midrule
% \eba-Ind & 55.7 & 49.3 \\
% \eba & \textbf{60.0} & \textbf{76.9} \\
% \bottomrule
% \end{tabular}
% \caption{Performance comparison between \eba \ emplying independent document selection model (\eba-Ind) and employing the joint document selection model on HotpotQA.}
% \label{tab:parallel_sequential}
% \end{table}
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{ccrrrr}
% \toprule
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{Prec} & \multicolumn{1}{c}{Rec} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} \\ \midrule
% \multirow{2}{*}{Comparison} & \eba-Ind & \textbf{83.2} & \textbf{76.5} & \textbf{57.8} & \textbf{78.9} \\
%  & \eba & 82.2 & 75.9 & \textbf{57.8} & 78.1 \\ \midrule
% \multirow{2}{*}{Bridge} & \eba-Ind & 60.5 & 52.1 & 17.8 & 55.2 \\
%  & \eba & \textbf{77.7} & \textbf{67.1} & \textbf{38.0} & \textbf{71.0} \\
% \bottomrule
% \end{tabular}
% \caption{Rationale selection performance broken down by different types of reasoning.}
% \label{tab:breakdown}
% \end{table}
\begin{table}[t]
\centering
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{c}{Sent F1} & \multicolumn{1}{c}{Doc F1} & \multicolumn{1}{c}{Ans F1} \\ \midrule
\multirow{2}{*}{Comparison} & \eba-Ind & \textbf{78.9} & \textbf{92.9} & 64.8 \\
 & \eba & 78.1 & 91.1 & \textbf{69.7} \\ \midrule
\multirow{2}{*}{Bridge} & \eba-Ind & 55.2 & 68.6 & 71.6 \\
 & \eba & \textbf{71.0} & \textbf{87.3} & \textbf{75.7} \\ \midrule
\multirow{2}{*}{Combined} & \eba-Ind & 60.0 & 73.4 & 69.1 \\
 & \eba & \textbf{72.5} & \textbf{88.0} & \textbf{73.5} \\
\bottomrule
\end{tabular}
\caption{Rationale selection performance broken down by different types of reasoning.}
\vspace*{-10pt}
\label{tab:breakdown}
\end{table}
\section{Analysis}
%\paragraph{Comparing Sequential Reasoning to Parallel Reasoning}
\paragraph{Document Dependencies}
% Here, we investigate whether it is necessary to predict the second document based on the first document.
\eba \ explicitly models the dependencies between documents for multihop reasoning.
We consider independent document selection~\footnote{We provide the detail of training and testing independent document selection model in Appendex~\ref{sec:ind-doc-select}.} to see whether this dependencies is necessary on the HotpotQA dataset.
%We test these two types of reasoning on the HotpotQA dataset.
%We implement parallel reasoning by choosing documents independently; that is, in the context of HotpotQA, each of the two documents are selected without taking into account the other document.
%For parallel reasoning, we train a different latent-variable model that makes an independence assumption between documents and selects the two documents by taking $\argmaxB_{d_1, d_2} P(d_1) P(d_2)$ with $d_1 \neq d_2$.
%For independent document selection, we train a different document selection model that assumes $p(\bm{d} \mid x) = \prod p(d_i \mid x)$.
%As HotpotQA has two relevant document, at test time we select the documents via $\argmaxB_{d_1, d_2} p(d_1\mid x) p(d_2 \mid x)$ with $d_1 \neq d_2$.
%We compute the document accuracy (i.e., both documents being predicted correctly) and answer EM.
%We summarize the results in Table~\ref{tab:parallel_sequential}: even though both sequential reasoning and parallel reasoning can correctly predict answers for a similar number of examples, sequential reasoning correctly predicts almost twice as many documents.
% Table~\ref{tab:parallel_sequential} summarizes answer EM and document EM. 
% Both independent document selection model and joint document selection model lead to similar performance in predicting answers.
%They also produce similar accuracy in predicting one document correctly.
% However, the joint document selection model is substantially better at identifying both documents.

To understand how document modeling impact rationale selection performance, we break the performance down by the reasoning types proposed in~\citet{yang-etal-2018-hotpotqa}: comparison-based reasoning and bridge-based reasoning.
In comparison-based reasoning, relevant documents independently contribute to the answer, whereas for bridge-based reasoning, relevant documents require connections to previously selected documents.
Table~\ref{tab:breakdown} summarizes answer F1 scores, document F1 scores, and sentence F1 scores.
While \eba-Ind is slightly better at comparison-based reasoning than the joint model, it fails at bridge-based reasoning; this result thus confirms the necessity of modeling the dependency between documents.
We also note that \eba-Ind and \eba \ have similar performance in predicting answers, but the gap between how accurate they select rationales is large, suggesting that \eba-Ind often derives answers with wrong reasoning.
Overall, \eba \ is better than \eba-Ind \ at both predicting answers and selecting rationales.

In addition to the quantitative analysis, we also qualitatively compare the two models in Figure~\ref{fig:qualitative}.
When considering paragraphs independently, documents A and C share the most entities with the question (i.e., Copsi, earl of Northumbria, and Two Rivers), so they are more likely to lead to the answer.
However, the correct documents are A and B. Deriving B not only depends on the question but also further requires knowing the information from A. Therefore, while having the independent document selection model can improve efficiency because it only performs one-step reasoning, the joint document selection model is necessary when reasoning steps depend on one another.

\begin{figure}[!t]
    \framebox{
    \parbox{0.45\textwidth}{
    \small
    \textbf{Q:} When \entity{Copsi} was made \entity{earl of Northumbria} he went to reside in a town at the confluence of which \entity{two rivers}?\noindent \smallskip \newline
    \textbf{Document A, Copsi:} \newline
    \entity{Copsi} survived Tostig's defeat at Stamford Bridge, and when William the Conqueror prevailed at Hastings he travelled, in March 1067, to pay William homage at Barking (where William was staying while his tower was being constructed in London). \support{In return, William made \entity{Copsi earl of Northumbria} and sent him back to York.}\newline
    \textbf{Document B, York:} \newline
    \support{York is a historic walled city at the confluence of the rivers Ouse and Foss in North Yorkshire, England.} The municipality is the traditional county town of the historic county of Yorkshire to which it gives its name.\newline
    \textbf{Document C, Two Rivers Press:} \newline
    \entity{Two Rivers} Press is an independent publishing house, based in the English town of Reading. Two Rivers Press was founded in 1994 by Peter Hay (1951–2003).\smallskip \newline
    \textbf{A:} Ouse and Foss}
    }
    \caption{A HotpotQA example where there is a dependency between two supporting documents, and thus selecting the second document independent of the first one results in insufficient information. Correct rationale is highlighted in \support{blue italics}. Entity overlaps between questions and documents are in \entity{red boldface}. \eba-Ind's predicted Documents B and C, whose reasoning remains at the surface level as they share the most entities with the question. \eba \ predicted Documents A and B, which demonstrates its ability of understanding dependency between documents.} \label{fig:qualitative}
\end{figure}
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{lcc}
% \toprule
% % & \multicolumn{1}{l}{\textbf{R{\noindent \color{green} \cmark }A{\noindent \color{green} \cmark}}} & \multicolumn{1}{l}{\textbf{R{\noindent \color{green} \cmark}A{\noindent \color{red} \xmark}}} & \multicolumn{1}{l}{\textbf{R{\noindent \color{red} \xmark}A{\noindent \color{green} \cmark}}} & \multicolumn{1}{l}{\textbf{R{\noindent \color{red} \xmark}A{\noindent \color{red} \xmark}}} & \multicolumn{1}{l}{\textbf{A}{\noindent \color{green} \cmark}} \\ 
% % & $\uparrow$ & $\uparrow$  & $\downarrow$ & $\downarrow$ & $\uparrow$ \\ \midrule
% % \textbf{Parallel} & 20.7\% & 19.3\% & 31.3\% & 28.7\% & 52.0\% \\
% % \textbf{Sequential} & 40.9\% & 29.8\% & 12.6\% & 16.7\% & 53.5\% \\
%  & Right Answers & Right for Right Reasons\\ \midrule
% Parallel & 3850 & 1533 \\
% Sequential & 3961 & 3029 \\
% \bottomrule
% \end{tabular}
% \caption{Comparison between parallel reasoning and sequential reasoning on the number of examples that are predicted correctly and the number of examples that are predicted correctly for the right reasons on the HotpotQA test set.}
% \end{table}
% \begin{figure}[!t]
%     \framebox{
%     \parbox{0.45\textwidth}{
%     \small
%     \textbf{Q:} Brown State Fishing Lake is in a country that has a population of how many inhabitants? \noindent \smallskip \newline
%     \textbf{Document A, Osage State Fishing Lake:} \newline
%     Osage State Fishing Lake is located in northern Osage County, Kansas. It is a mile east of US 75. Scranton, Kansas, is to the lake's northwest and Overbrook, Kansas, is to the northeast.\newline
%     \textbf{Document B, Brown State Fishing Lake:} \newline
%     \support{Brown State Fishing Lake (sometimes also known as Brown State Fishing Lake And Wildlife Area) is a protected area in Brown County, Kansas in the United States.} The lake is 62 acres in area and up to 13 feet deep. The area was formerly known as Brown County State Park, and is 8 miles east of Hiawatha, Kansas.\newline
%     \textbf{Document C, Brown County, Kansas:} \newline
%     Brown County (county code BR) is a county located in the northeast portion of the U.S. state of Kansas. \support{As of the 2010 census, the county population was 9984.} Its county seat and most populous city is Hiawatha.\smallskip \newline
%     \textbf{A:} 9984}
%     }
%     \caption{} \label{fig:analysis}
% \end{figure}
\begin{table}[t]
\centering
\small
% \begin{tabular}{lcrr}
% \toprule
% Answer Model & Type & \multicolumn{1}{l}{Sent F1} & \multicolumn{1}{l}{Ans F1} \\ \midrule
% \textit{Explainable}&&&\\
% BART-base & Generate & 48.4 & 74.3 \\
% BART-large & Generate & \textbf{52.5} & 74.1 \\
% DistilBERT & Classify  & 14.8 & 75.3 \\
% RoBERTa-base & Classify & 20.0 & 79.9\\
% RoBERTa-large & Classify & 15.9 & \textbf{82.4} \\ \midrule
% \textit{Blackbox}&&&\\
% RoBERTa-large & Classify & - & \textbf{84.6} \\
% RoBERTa-large (w/o $D$) & Classify & - & 82.1 \\
% \bottomrule
% \end{tabular}
\begin{tabular}{lcccc}
\toprule
Answer Model & Pred Type & \multicolumn{1}{l}{FEVER} & \multicolumn{1}{l}{MultiRC} \\
&& \multicolumn{2}{c}{\textbf{Sent F1}} \\
\midrule
BART & Generate &81.5 & 48.4 \\
% BART-large & Generate & 80.8 &\textbf{52.5} \\
% DistilBERT & Classify & 80.5 & 14.8 \\
RoBERTa & Classify & 82.0 & 20.0\\
% RoBERTa-large & Classify & 81.2 & 15.9 \\
\bottomrule
\end{tabular}
\caption{Comparison on sentence F1 scores between different parameterization choices of $P(y\mid\bm{z}, x)$.
%-- one predicts answers with both questions and documents, while the other predicts answers with the questions only.
}
\label{tab:answer_parameterization}
\end{table}

\begin{figure}[]
    \framebox{
    \parbox{0.45\textwidth}{
    \small
    \textbf{Q:} What did the judge tell Mr. Thorndike about the law? \noindent \smallskip \newline
    \textbf{A1:} {\color{blue}\textit{Cannot be swayed by wealth or political influences.}}\newline
    \textbf{A2:} {\color{blue}\textit{The law is not vindictive.}}\newline
    \textbf{A3:} {\color{blue}\textit{It was not vindictive.}}\newline
    \textbf{A4:} It was unjust.\newline
    \textbf{A5:} It was vindictive.\newline
    \textbf{A6:} {\support{The judge told Mr. Thorndike that the law is not vindictive. He said the law only wishes to be just. Judge said the law cannot be swayed by wealth or political influences.}}
    }
    }
    \caption{A test example from MultiRC that can be answered with commonsense reasoning and thus requires no accompanying documents. Correct answers are highlighted in \support{blue italics}.}
    \vspace*{-10pt}
    \label{fig:multirc_commonsense}
\end{figure}
%\paragraph{Obtaining Richer Learning Signals with Encoder-decoder Models}
\paragraph{Role of Answer Generation}
\eba \ uses a generative model (BART) to parameterize $p(y\mid \bm{z}, x)$. An alternative approach would be to use a classification model such as RoBERTa~\cite{DBLP:journals/corr/abs-1907-11692} to predict answers for FEVER and MultiRC (HotpotQA requires a generative model). 

Interestingly, Table~\ref{tab:answer_parameterization} shows the choice of answer model significantly impacts the ability of \eba \ to learn a rationale model. 
On FEVER, where claims cannot be verified without the corresponding rationales, BART and RoBERTa perform similarly. However, on MultiRC, where questions can often be answered without information in accompanying documents, the best Generative model outperforms the best Classification model by over 32 sentence F1 points.

% In \eba, the learning signal for identifying rationales comes from answer supervision. 
% % -- if conditioning on a rationale makes an answer become more likely, that rationale will be upweighted during training.
% % Thus, for \eba \ to be functioning effectively, accurate estimation of the answer model $p(y\mid \bm{z}, x)$ is crucially important.
% Here, we show that different parameterization choices for $p(y\mid \bm{z}, x)$ can play a key role in selecting rationales when datasets. 

% are poorly constructed with shortcuts (i.e., answers can directly be derived from questions without rationales).
% Specifically, using sequence-to-sequence models for the parameterization can provide a richer learning signal for the intermediate steps than using encoder-only models such as BERT~\cite{devlin-etal-2019-bert}.

%Although parameterizing the answer model $p(y\mid \bm{z}, x)$ with RoBERTa better predicts answers than with BART,
% We take RoBERTa~\cite{DBLP:journals/corr/abs-1907-11692} as the encoder-only model and BART as the sequence-to-sequence model, and we report the results on FEVER and on MultiRC in Table~\ref{tab:answer_parameterization}.


%To understand why RoBERTa models can ignores the rationales to predict answers, we perform standard fine-tuning on a RoBERTa model to predict answers based on questions $x$ alone.
%Table~\ref{tab:answer_parameterization} shows that predicting answers with and without documents $D$ only results in a minor difference; in other words, in many examples the questions alone provide enough discriminative features for answer predictions.
%This dataset flaw can also explain why the sentence F1 scores on MultiRC are the lowest across all three datasets in Section~\ref{sec:results}.

% We hypothesize that when answers can be directly derived from the questions alone, classification models ignore the rationales.
%and still be accurate at predicting the answers (achieving similar answer F1 scores as those of BART models).
%We inspect the test examples in MultiRC and find that many of their questions can be answered without further evidence.
Figure~\ref{fig:multirc_commonsense} shows an example of such a question where the answers can be guessed by the classification model using commonsense knowledge to reason about law.
% Despite this dataset issue, BART can still leverage the answer annotations to learn the intermediate reasoning steps.
Generative models need to assign a high probability to every token in the answer, and we hypothesize that they make better use of the answer supervision.

\paragraph{Speed evaluation.}
\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
 & \eba & \textsc{Faithful} & Ratio \\ \midrule
Training & 11,544.2 & 444.0 & 26 \\
Inference &    39.0 & 3.9   & 10 \\
\bottomrule
\end{tabular}
\caption{Runtime comparison (in seconds). \eba \ uses 80 rationale samples at training time, and the argmax rationale at inference.}
\label{tab:overhead}
\end{table}

While \eba \ obtains strong sentence F1 scores,
training is more expensive because the model must consider a set of rationales for every example.
In particular, the answer model $p(y\mid \bm{z}, x)$ must be run for \emph{every} sampled $\bm{z}$ for each training example.
At inference, the answer model requires only a single evaluation of $p(y\mid \bm{z}, x)$ for $\argmaxB_{\bm{z}} p(\bm{z}\mid x)$.
%The superior performance of \eba \ comes with a cost.
%The main source of overhead is from the computation in the answer model. 
%At training, the answer model requires computing $p(y\mid \bm{z}, x)$ for \emph{every} sampled $\bm{z}$.
%At inference, the answer model requires computing $p(y\mid \bm{z}, x)$ for $\argmaxB_{\bm{z}} p(\bm{z}\mid x)$.
We empirically measure the runtime overhead of \eba \ compared to \textsc{Faithful} on MultiRC, using 80 samples of $\bm{z}$ at training time.
We report the total training time and inference time in Table~\ref{tab:overhead}.
%\eba \ takes 25x more time to train and 9x more time to make inference.
Compared to \textsc{Faithful}, \eba \ takes longer to train and to predict.
%We note that because \eba \ only conditions on questions to select rationales, it avoids computing the posterior distribution of $\bm{z}$, thus making the inference overhead much less than training overhead.

==> exNLP_acl2023 (Copy)/conclusion.tex <==
\section{Conclusion}
We present \eba, a probabilistic, principled approach for explainable multi-hop reasoning without rationale supervision.
\eba \ explicitly models multi-hop reasoning by considering the dependency between documents and between sentences within a document.
Experimental results demonstrate that \eba \ outperforms other state-of-the-art methods that do not rely on rationale labels.

==> exNLP_acl2023 (Copy)/introduction.tex <==
\section{Introduction}
% Large language models have achieved tremendous success on a wide range of natural language processing (NLP) tasks, even in the few-shot or zero-shot setting~\cite{brown2020language,chowdhery2022palm}.
% However, these models are black-box, making it difficult to evaluate their trustworthiness~\cite{jia-liang-2017-adversarial}.
% Thus, relying on these models' predictions to make critical decisions can lead to serious harm if the predictions are right for the wrong reasons.
% Understanding models' predictions is crucial to safely deploying real-world NLP systems.
Multi-hop reasoning is an important capability for any intelligent machine comprehension system.
Question answering (QA) is a common application for evaluating a system's ability to reason across multiple steps~\cite{geva-etal-2021-aristotle,yang-etal-2018-hotpotqa,welbl-etal-2018-constructing}.
Large language models have achieved tremendous success on challenging QA tasks, even in the few-shot setting~\cite{wei2022chain}.
%However, \citet{chen-durrett-2019-understanding} demonstrate that these models get around multi-hop reasoning by performing shallow pattern matching.
%Worse, they can even derive answers by exploiting reasoning shortcuts~\cite{jia-liang-2017-adversarial}.
However, \citet{min-etal-2019-compositional} and \citet{chen-durrett-2019-understanding} demonstrate that these models, in reality, often bypass multi-hop reasoning by performing shallow pattern matching, resulting in poor generalization ability~\cite{tang-etal-2021-multi}. 
%Building QA systems that can reliably perform multi-hop reasoning requires understanding the series of steps the systems follow to derive the answers.
To avoid predictions made from such reasoning shortcuts, it is important to understand the series of steps the systems follow to derive the answers.

%This work explores the challenge of building explainable multi-hop QA systems.
This work explores the challenge of building explainable multi-hop QA systems, which, in addition to predicting an answer, also identify a \emph{rationale} -- the set of sentences that lead to the answer.
Depending on task specifications, the rationale can be within a single document, or span across multiple documents.
%When performing multi-hop reasoning across multiple documents, researchers identified two difficult, but important reasoning types -- comparison-based reasoning and bridge-based reasoning~\cite{yang-etal-2018-hotpotqa,min-etal-2019-multi,nishida-etal-2019-answering,fu-etal-2021-decomposing-complex}.
%As shown in Figure~\ref{fig:overview}, relevant documents in comparison-based reasoning can be identified independently, whereas relevant documents in bridge-based reasoning have to be identified sequentially.
%Therefore, being able to capture the dependency between documents is key to performing bridge-based reasoning.
Explainable multi-hop QA has been extensively studied in the supervised setting, where both rationale annotations and answer annotations are given.
These approaches either apply multi-task loss functions~\cite{joshi-etal-2020-spanbert,groeneveld-etal-2020-simple,deyoung-etal-2020-eraser} or design specialized network architectures~\cite{tu-etal-2019-multi,fang-etal-2020-hierarchical}.
However, having access to rationale annotations is a strong assumption.
In practice, they are expensive to collect~\cite{geva-etal-2021-aristotle}, less available than answer annotations~\cite{welbl-etal-2018-constructing}, and can suffer from low agreement rates between annotators~\cite{zhang-etal-2020-winowhy}.
%Here, hops are defined at the sentence level; if a question requires reasoning over multiple sentences to reach the answer, then we consider it to be a multi-hop QA problem, and the set of sentences is called a \emph{rationale}.
%We identify two issues that make building explainable multi-hop QA systems a particularly challenging problem.
%First, rationale annotations are not always available can be expensive to collect: the cost of annotating one example in StrategyQA is four dollars~\cite{geva-etal-2021-aristotle}.
%Human explanations can also be subjective and introduce biases: the agreement rate between annotators on what the correct rationales are can be low~\cite{zhang-etal-2020-winowhy}.
%The second issue relates to efficiency -- there are exponentially many possible rationales, and naively score every rationale individually is computationally intractable.
%Common ways of interpreting models' answer predictions include generating free-form explanations and highlighting relevant sentences~\cite{wiegreffe2021teach}.
%While free-form texts provide more expressive, concise explanations~\cite{inoue-etal-2021-summarize},  such approaches are prone to producing explanations that are self-contradictory for the same answer \cite{camburu-etal-2020-make}.
%The alternative approach of selecting sentences for rationales is faithful by construction,
%and therefore the focus of this work.
%To stay faithful to the supporting documents, selecting sentences as rationales for answer predictions is thus preferred.

% The most prevalent approach for learning an explainable multi-hop QA system is to directly supervise sentence-level rationales, by either applying multi-task loss functions~\cite{joshi-etal-2020-spanbert,groeneveld-etal-2020-simple,deyoung-etal-2020-eraser} or specialized network architectures~\cite{tu-etal-2019-multi,fang-etal-2020-hierarchical}.
% Though these methods achieve state-of-the-art performance on predicting answers and relevant sentences, one major drawback is that they produce answers independent from rationales.
%\justin{trying to think of a more convincing way of describing the flaw. without constraining the answer generating process, the same pitfalls of unexplainable models exist: shortcuts / incorrect reasoning.}
%In other words, without conditioning the answers on the predicted rationales, one still fails to evaluate the trustworthiness of such systems.
% In other words, without conditioning the answers on the predicted rationales, one fails to recognize whether correct predictions are made from reasoning shortcuts.
% Furthermore, relying on sentence annotations can introduce following issues.
% First, such annotations are not always available, and they can be expensive to collect: the cost of annotating one example in StrategyQA is four dollars~\cite{geva-etal-2021-aristotle}.
% Secondly, explanations are subjective: the agreement rate between annotators on what the correct rationales are can be low~\cite{zhang-etal-2020-winowhy}.

% Recent interest has thus shifted to developing semi-supervised or unsupervised approaches for learning explainable multi-hop QA systems.
% \citet{chen2019multi} leverage entity taggers to build silver reasoning chains used for rationale supervision.
% However, they are criticized for exploiting heuristics specific to individual datasets.
% \citet{glockner-etal-2020-think,atanasova2022diagnostics} design loss functions to enforce a number of properties on selected rationales.
% These methods, nevertheless, do not scale to handle multiple documents.

%Unsupervised approaches to QA rationales can eliminate the need for annotations.
Researchers have thus explored approaches that do not require rationale annotations~\citep{NEURIPS2020_6b493230,glockner-etal-2020-think,atanasova2022diagnostics}.
% \citet{atanasova2022diagnostics} classify whether each sentence is included in the rationale independently.
% \citet{glockner-etal-2020-think} predict an answer from every sentence pair and take the sentence pair that can most confidently predict the answer as the rationale.
However, these previous approaches limit their reasoning to information from 1 or 2 sentences, and so they cannot be applied in \textit{multi-hop} scenarios, i.e. QA tasks that require making connections between several pieces of information across sentences and across documents. Additionally, these methods are either restricted to only work for multiple-choice QA, or restricted to only produce rationales at the document level but not at the sentence level.
%Additionally, the loss functions of \citet{atanasova2022diagnostics} and \citet{glockner-etal-2020-think} assume that answers are categorical, so they do not work for abstractive or extractive QA datasets such as HotpotQA~\cite{yang-etal-2018-hotpotqa}.
% Because , they do not have the modeling capacity to perform multi-hop reasoning.
%\citet{chen2019multi} leverage entity taggers to build silver reasoning chains used for rationale supervision.
%However, this approach is specific to datasets constructed with entity linking and thus cannot be generalized to other types of reasoning.
%However, this approach is specific to perform bridge-based reasoning and cannot be generalized to perform comparison-based reasoning.
%However, they are criticized for overfitting specific datasets that are constructed with entity linking and thus cannot be generalized to other types of reasoning.
%\citet{glockner-etal-2020-think,atanasova2022diagnostics} design loss functions to enforce a number of properties on selected rationales in an unsupervised manner.
%These methods, nevertheless, treat multiple documents as a single one; for this reason, they become inefficient to apply when the number of documents becomes large.
%To summarize, none of the existing solutions are satisfactory.
%\citet{glockner-etal-2020-think,atanasova2022diagnostics} develop general unsupervised approaches that do not rely on any dataset heuristic.
%\citet{glockner-etal-2020-think} assume the sentences in a rationale are fully dependent on each other.
%This expensive modeling choice prevents them from scaling up to identifying rationales that have more than two sentences.
%\citet{atanasova2022diagnostics}, falling on the other extreme, chooses each sentence in the rationale independently, and this over-simplifying independence assumption results in predicting answers with many reasoning shortcuts.
%These methods, nevertheless, either selects each sentence in the rationale independently; for this reason, they become inefficient to apply when the number of documents becomes large.
%\citet{glockner-etal-2020-think} and \citet{atanasova2022diagnostics} design new loss functions for training explainable multi-hop QA systems without rationale supervision.
%This approach, however, cannot handle cases where rationales span across multiple documents.
%Therefore, none of the existing solutions are satisfactory.

%This work improves upon previous systems by identifying a better trade-off between accuracy and efficiency. We propose \fulleba \ (\eba), an approach to multi-hop QA that treats sentence-level rationales as a latent variable. \eba \ relies only on gold answers and does not require supervision over rationales, making it applicable to any multi-hop QA task with gold answers. Figure~\ref{fig:overview} presents an overview of the three stages of \eba:
%First, \eba \ selects the relevant documents given the question.
%Next, within each of the selected documents, \eba \ selects a subset of sentences.
%Finally, \eba \ generates an answer given all selected sentences across all documents.
We propose \fulleba \ (\eba), a principled, probabilistic approach for training explainable multi-hop QA systems without rationale supervision.
%\eba \ treats documents and rationales as latent variables and explicitly models multi-hop reasoning by considering the dependency both between documents and between sentences within a document.
\eba \ overcomes the two-sentence limitation of previous methods by directly reasoning about rationales as \textit{sets} of sentences, while also extending rationale prediction to the multi-document setting.
%\eba \ performs multi-hop reasoning by explicitly modeling the relationship between documents and between sentences within each document.
We show an overview of \eba \ in Figure~\ref{fig:overview}.
\eba \ leverages the naturally hierarchical structure of text and proceeds in three stages -- it first selects the relevant set of documents given the question (Hop); then, it selects a subset of sentences within each of the relevant documents and collects them together (Union); finally, it generates an answer via a seq2seq model with all the collected sentences (Generate).
%\eba \ treats a rationale as a latent variable and explicitly models the dependency between documents.
%Because of this expressive modeling capacity, \eba \ can perform both comparison-based and bridge-based reasoning shown in Figure~\ref{fig:overview}.
% Further, multi-hop reasoning also requires understanding the interaction between sentences (e.g., resolving coreferences among multiple sentences).
% Therefore, \eba \ also explicitly models the full dependency between sentences within a document.
%Based on a question, \eba \ identifies the documents from which a reasoning chain can be formed to derive the answer.
The key to multi-hop reasoning in \eba \ is modeling each selection as an explicit distribution over sets.
A probabilistic set distribution compares non-contiguous and variable size rationales, affording \eba \ flexibility for rationale selection.

%We overcome two challenges when training \eba.
Training a set-prediction model quickly becomes intractable as the size increases.
We make two algorithmic choices that lead to tractable training for \eba.
Treating rationales as a latent variable requires \eba \ to marginalize over all possible rationales, leading to an intractable learning objective.
%We solve this by trading off accuracy for efficiency:
%we utilize efficient sampling techniques and introduce conditional independence assumptions into the model.
\eba \ overcomes this issue by performing sampling in a hierarchical way -- it first identifies the most promising documents and then the most promising sentences within those documents.
Second, multi-hop QA often involves reasoning over long documents,
which is challenging due to the computational complexity of encoding long documents with neural models such as transformers. 
%and encoding such long documents with transformer models has a quadratic complexity with regards to the number of tokens.
%To make this encoding efficient, \eba \ adopts ideas from SentenceBERT~\cite{reimers-gurevych-2019-sentence}, which leverages computation in the embedding space.
To make this encoding efficient, \eba \ performs computation in the embedding space.
%we again trade off accuracy for efficiency by adopting ideas from SentenceBERT~\cite{reimers-gurevych-2019-sentence},
%\justin{might be confusing for readers}
% Second, since a rationale is a collection of sentences, we must do something with the rationale encoding.
% We overcome this by using an efficient encoding of documents that something.

% This work aims to improve upon the previous systems by better trading off between accuracy and efficiency.
% To this end, we propose an unsupervised approach, \fulleba \ (\eba), for multi-hop QA that treats sentence-level rationales as a latent variable.
% Because marginalizing this latent variable out does not require any annotation for the true rationale, \eba \ allows us to fit our system to any multi-hop QA task with only the gold answers.
% Figure~\ref{fig:overview} presents an overview of \eba, which proceeds in three stages.
% % We assume each multi-hop QA task comes with a pre-specified number of relevant documents $m$.
% In the first step, \eba \ selects relevant documents.
% Next, within each of the selected documents, \eba \ scores sentence subsets.
% Finally, \eba \ generates an answer with an encoder-decoder language model such as BART~\cite{lewis-etal-2020-bart}.
% In the event of performing multi-hop reasoning over a single document, the first step will be skipped.

% \eba \ makes the following three design choices to trade off between accuracy and efficiency.
% %Our proposed method is principled -- it first generates a prior distribution over all possible rationales given the question alone, and it then produces an answer based only on the selected rationale.
% %Our method proceeds in two stages for selecting rationales -- it first identifies which documents are relevant to the question, and then chooses sentences from those documents.
% First, we make careful modeling choices: when selecting a document at stage 1, we take into account other documents; however, when selecting a set of sentences within a document at stage 2, we do not consider the sentences in other documents.
% These modeling choices allow \eba \ to both consider the dependency between documents and prune the rationales that have sentences in unrelated documents.
% Secondly, for some of the modeling choices that are still expensive because we need to account for the sequential nature of multi-hop reasoning, we strive for a cheap way to parameterize those models.
% Last but not least, while the objective function associated to our modeling choices is intractable to compute, we approximate it with efficient sampling techniques. 
%Finally, although it is computationally expensive to train a multi-hop QA system with our method, it incurs little overhead at inference time.
%This is because evaluating the trustworthiness of a system only concerns prior rationales but not posterior rationales, which requires marginalizing over all possible answers.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/Bridge.pdf}
    %\caption{An overview for the proposed approach, \eba, which proceeds in three stages. Here, we assume there are two relevant documents; i.e., there are two relevant documents to the question. Stage 1 will be skipped when performing multi-hop reasoning over a single document.}
    \caption{
    An overview of \eba, which proceeds in three stages. \textbf{Hop} explicitly considers all possible document sets and selects the most likely document set, \textbf{Union} explicitly considers all sentence subsets and chooses the most likely sentence subset within each selected document, and \textbf{Generate} combines the chosen sentence subsets and generates an answer.
    %An overview of \eba, which models the relations between documents and between sentences within a document.
    %\eba \ is a generative system that first selects a set of relevant documents, then selects a rationale (subset of sentences) from those documents, and finally generates an answer.
    %\eba \ can capture relationships between documents, for instance in this example possibly related sentences (red) in different documents.
    %The proposed approach, \eba, performs both comparison-based and bridge-based multi-hop reasoning over documents without rationale supervision. 
    %Multi-hop reasoning can be comparison-based or bridge-based.
    %Two example reasoning types for multi-hop QA are comparison-based or bridge-based.
    %Given the question, the former identifies two documents in parallel, and the latter identifies two documents sequentially.
    %The proposed approach, \eba, can handle both reasoning types.
    %Based on a question, \eba \ selects documents that can form a reasoning chain to the answer.
    }
    \label{fig:overview}
\end{figure}

% Recently, \citet{wei2022emergent} and \citet{chung2022scaling} show that language models of larger size have better reasoning abilities.
% We note that \eba \ is orthogonal to the development of these models.
% \eba \ is a way to impose constraints on the process of multi-hop reasoning, and it can benefit from using larger, more expressive language models.

We empirically evaluate \eba \ on three different multi-hop QA datasets: HotpotQA~\cite{yang-etal-2018-hotpotqa}, MuSiQue~\cite{trivedi2021musique}, FEVER~\cite{deyoung-etal-2020-eraser}, and MultiRC~\cite{deyoung-etal-2020-eraser}.
Results show that, for both selecting rationales and predicting answers, \eba \ is better than a number of state-of-the-art semi-supervised and unsupervised methods~\cite{chen2019multi,NEURIPS2020_6b493230,glockner-etal-2020-think,atanasova2022diagnostics} on all of the datasets.
We also demonstrate that \eba \ combined with larger language models consistently produces better performance.
We then analyze performance according to different types of multi-hop reasoning and show that by explicitly modeling multi-hop reasoning, \eba \ achieves a large improvement on the reasoning type that requires bridging entities.
% Finally, we perform further analysis to understand which components of \eba \ are key to accurate rationale selection.
%We then perform analysis to show our modeling choice is better than the alternatives.
%Specifically, when the dependency between documents are removed at stage 1, not only does the accuracy for rationale selection drop, but also the model predicts correct answers for the wrong reasons.
%Additionally, we show that using encoder-decoder models to produce answers can provide better learning signal for rationale selection than encoder-only models.
% Additionally, we demonstrate how explainability brings insights into datasets; for example, \eba \ identifies examples in HotpotQA that do not need multiple documents to derive the correct answers.

==> exNLP_acl2023 (Copy)/method.tex <==
\section{Generative Multi-Hop QA}
\begin{figure}
    \centering
    \small
    \framebox{
    \parbox{0.45\textwidth}{
    \small
    $x$: Emily Beecham is best known for her role in a television series whose second season premiered on what date? \noindent \smallskip \newline
    $d_1$: \textbf{[1]} \support{\underline{Emily Beecham} is an English-American actress.} \textbf{[2]} \support{\underline{She} is best known for her role in the AMC television series ``\bridge{Into the Badlands}''}  \textbf{[3]} In 2011, she received the Best Actress award at the London Independent Film Festival.\smallskip \newline
    $d_2$: \textbf{[4]} \support{\underline{\bridge{Into the Badlands}} is an American television series that premiered on AMC November 15, 2015} \textbf{[5]} The series features a story about a warrior and a young boy who journey through a dangerous feudal land together seeking enlightenment. \textbf{[6]} \support{AMC renewed \underline{the show} for a 10-episode second season, which premiered on March 19, 2017.} \textbf{[7]} On April 25, 2017, AMC renewed the series for a 16-episode third season.'\smallskip \newline
    $\bm{z}$: [1], [2], [4], [6] \smallskip \newline
    $y$: March 19, 2017}
    }
    \caption{A QA example. The rationale $\bm{z}$ used to derive the answer is highlighted in \support{blue italics}, the document-level interaction is highlighted in \bridge{red boldface}, and the sentence-level interaction (i.e., coreference resolution) is highlighted in \underline{underline}. \eba \ models dependencies both between documents and between sentences within a document, thus being equipped with the capacity to perform multi-hop reasoning.}
    \label{fig:multihop_example}
\end{figure}

% \begin{figure}[t]
%   \begin{center}
%   \scalebox{.85}{
%     \begin{tikzpicture}
%     \node[obs] (x) {$x$};
%     \node[latent, right=of x] (d) {$d_1$};
%     \node[latent, below=of d] (dd) {$d_2$};
%     \node[latent, right=of d] (z) {$\bm{z}_1$};
%     \node[latent, right=of dd] (zz) {$\bm{z}_2$};
%     \node[obs, right=of z] (y) {$y$};
%     \edge {x} {d};
%     \edge {x} {dd};
%     \draw[->] (x) to[bend left] (z);
%     \draw[->] (x) to[bend left] (y);
%     \edge {x} {zz};
%     \edge {d} {dd};
%     \edge {d} {z};
%     \edge {dd} {zz};
%     \edge {z} {y};
%     \edge {zz} {y};
%     \end{tikzpicture}
%     }
%   \end{center}
% \caption{The graphical model for the data generating process for multi-hop QA with two relevant documents.}
% \label{fig:generative2}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% \scalebox{.85}{
%     \begin{tikzpicture}
    
%     \node[latent] (d) {$d_i$};
%     \node[latent, right=of d] (z) {$\bm{z}_i$};
%     \node[obs, right=of z] (y) {$y$};
%     \node[obs, left=of d] (x) {$x$};

%     \factor[left=of d] {d-f} {} {} {};
%     \factor[right=of d] {z-f} {} {} {};
%     \factor[right=of z] {y-f} {} {} {};

%     \factoredge[-] {x} {d-f} {d};
%     %\edge[-] {x} {d-f}
%     \factoredge[->] {d} {z-f} {z};
%     \factoredge[->] {z} {y-f} {y};
%     \draw[-] (x) to[bend left=40] (z-f);    
%     \draw[-] (x) to[bend left=40] (y-f);
    
%     \plate {} {
%         (d)(z-f)(z)
%     } {$|\bm{d}|$}; 

%     \end{tikzpicture}
% }
% \end{center}
% \caption{The plated factor graph for the data generating process for multi-hop QA with $|\bm{d}|$ documents.
% %Plate factor graph alternative. The other diagram is inaccurate since document distribution is directly parameterized
% }
% \label{fig:generative2}
% \end{figure}

%Throughout the paper, we use uppercase letters to denote random variables and lowercase letters to denote specific values.
%In this paper, sets are bold and represented as binary vectors.
%An multi-hop QA example consists of a question $x$, a set of documents $\bm{d}$, and an answer $y$.
In the standard multi-hop QA setting, an example consists of a question $x$, a set of documents $D$, and an answer $y$.
Within $D$, some documents are relevant to the question, while the others are distractors. 
%Explainable multi-hop QA models first predict a rationale $\bm{z}$, a minimal set of sentences across the relevant documents.
Explainable multi-hop QA models predict a rationale $\bm{z}$, a minimal set of sentences across the relevant documents, in addition to predicting the answer $y$.
%Models must then derive the answer $y$ using information from only the rationale $\bm{z}$ and question $x$.
% We define hops at the sentence level; if a question requires reasoning over multiple sentences to reach the answer, then we consider it to be a multi-hop problem.
% For simplicity, we assume there are at most two documents relevant to a given question, $d_1$ and $d_2$.
% We further let $\bm{z}_1 \subseteq d_1$ and $\bm{z}_2 \subseteq d_2$ be the smallest subsets of sentences that contain enough information to answer the question $x$.
% $z_1$ and $z_2$ are combined to form a complete rationale $\bm{z}=(\bm{z}_1, \bm{z}_2)$.
%with associated rationales $\bm{z}=(\bm{z}_1, \bm{z}_2)$.
%Unless specified otherwise, we assume there are exactly two documents relevant to the question.
We show a multi-hop QA example (with distracting documents omitted) in Figure~\ref{fig:multihop_example}.

%We let $D_1$ and $D_2$ to be the first and the second relevant documents, respectively.
%Let $D_1$ and $D_2$ be two relevant documents, yielding a rationale $\bm{Z}=(\bm{Z}_1, \bm{Z}_2)$, $\bm{Z}_1 \subseteq D_1$ and $\bm{Z}_2 \subseteq D_2$.

\subsection{Model}

We propose the following generative model for multi-hop QA. Given the question $x$, we first select a subset of documents $\bm{d}=\{d_1,d_2,\ldots\}\subseteq D$. Next, within each document $d_i$, we select a subset of sentences $\bm{z}_i$. Finally, conditioned on the union of sentence sets from each document, $\bm{z}=\cup_i\bm{z}_i$, we generate an answer $y$. The only assumption we make in the model is that sentence sets are selected independently among documents.
Formally, we write the model as,
\begin{align}
    p(\bm{d}, \bm{z}, y \mid x) &= p(\bm{d} \mid x) \label{doc} \\
    &\quad \cdot \prod_{i} p(\bm{z}_i \mid d_i, x) \label{rationale} \\
    &\quad \cdot p(y\mid\bm{z}, x). \label{answer}
\end{align}
% Specifically, we treat the sentences and documents selected in the hops as latent variables, which, together with questions, lead to answers.
% In other words, answers are derived from questions and rationales in the relevant documents, but we only observe questions but the others.
% To model the influence of unobserved rationales on answers, we model them as a latent variable.
We refer to Eq.~\ref{doc} as the document set selection model, Eq.~\ref{rationale} as the sentence set selection model,
Eq.~\ref{answer} as the answer generation model.


% Formally, our generative process first chooses all relevant documents jointly given a question, $d_1,d_2 \mid x$.
% Choosing the coarse set of information jointly allows \eba \ to support both comparison-based reasoning and bridge-based reasoning,
% as it allows the model to ensure that all relevant facts have been gathered.
% We assume that documents contain disjoint information, which must be combined through either comparison or bridge reasoning.
% We can therefore make a conditional independence when choosing rationales given documents: $\bm{z_1} \mid d_1, x$ and $\bm{z}_2 \mid d_2, x$.
% Finally, we concatenate all rationales, combining their information to predict an answer $y \mid \bm{z}_1, \bm{z}_2, x$.
% This yields the joint distribution
% \begin{align*}
%     &p(d_1, d_2, \bm{z}_1, \bm{z}_2, y)\\
%     %= &P(D_1)P(D_2|D_1) \\
%     &= p(d_1, d_2)
%     p(\bm{z}_1|d_1)p(\bm{z}_2|d_2)
%     p(y|\bm{z}_1, \bm{z}_2),
% \end{align*}
% %Because every model conditions on $X$, we omit it for brevity.
% where we omit conditioning on $x$ (in every subexpression) for brevity, and will do so for the remainder of this work.

%Our probabilistic model places a distribution over $(d_1, d_2, \bm{z}_1, \bm{z}_2, y)$ and factorizes according to the three phases as follows:
%\begin{align*}
%    &p(d_1, d_2, \bm{z}_1, \bm{z}_2, y)\\
%    %= &P(D_1)P(D_2|D_1) \\
%    &= p(d_1, d_2)
%    \cdot p(\bm{z}_1|d_1)p(\bm{z}_2|d_2)
%    \cdot p(y|\bm{z}_1, \bm{z}_2),
%\end{align*}
%Because every model conditions on $X$, we omit it for brevity.
%where we omit $x$ for all brevity, as all distributions condition on it.
%Because of the expressivity of this probabilistic model, where documents are chosen in a joint manner,
%Due to the assumption that documents are chosen jointly,
%\eba \ supports both comparison-based reasoning and bridge-based reasoning \textcolor{red}{because}.
%We then discuss the parameterization of each model.

% \subsection{Parameterization}
% %We then discuss the parameterization of each model.
% In this section we discuss the parameterization of each conditional distrbution.

\paragraph{Document Set Selection}
%We would like to efficiently model important interactions between documents. 
We select a set of documents $\bm{d}$ by directly parameterizing a distribution over all valid document sets.
%We therefore model $p(\bm{d}\mid x)$ as
% Let $f: d_1 \times d_2 \rightarrow \mathbb{R}$ be a learnable document pair scoring function, which first computes an embedding for a document pair and produces a logit for the embedding.
We rely on a document set scoring function $f(\bm{d}, x)$, which captures both the relevance of
the document set $\bm{d}$ to the question $x$, as well as the dependencies among the documents in the set.
The document set selection model is given by
\begin{equation*}
    p(\bm{d} \mid x) \propto \exp(f(\bm{d}, x)).
\end{equation*}
%which is globally normalized over subsets of the document set $D$.
% This allows the model to capture complex dependencies between documents.
This distribution is globally normalized over all valid subsets of documents $D$,
requiring the evaluation of the document scoring function $f$ on all valid document subsets.
Document set validity is dataset specific, and is discussed in Section \ref{sec:experiments}.

% Computing an embedding for every pair of documents takes quadratic time.
% To reduce this computation to linear time, we combine two documents in the embedding space via Siamese networks~\cite{reimers-gurevych-2019-sentence}.
For efficiency, the document set scoring function $f$ first computes embeddings of each document in the set $\bm{d}$ independently, then combines them with a neural network (MLP).
Formally, let $\text{emb}: \mathcal{V}^* \rightarrow \mathbb{R}^n$ be an embedding function that maps a sequence of text to an $n$-dimension vector, where $\mathcal{V}$ is the vocabulary.
% Let $\text{e}_{d_1}=\text{emb}(d_1)$ and $\text{e}_{d_2}=\text{emb}(d_2)$, and $[\cdot]$ be a concatenation operator:
% \begin{equation*}
% \text{emb}([d_1, d_2]) \approx [\text{e}_{d_1},\text{e}_{d_2},|\text{e}_{d_1}-\text{e}_{d_2}|].
% \end{equation*}
% Let $\text{MLP}: \mathbb{R}^{3n} \rightarrow \mathbb{R}$ be a multilayer perceptron,
The document set scoring function is given by
\begin{equation*}
    %f(d_1, d_2, \ldots) = \text{MLP}(\text{emb}(d_1), \text{emb}(d_2), \ldots).
    f(\bm{d}, x) = \text{MLP}(\text{emb}(d_1,x), \text{emb}(d_2,x), \ldots).
\end{equation*}
%Note that $P(D_1, D_2)$ is normalized over all document pairs.
%In practice, $\text{emb}(\cdot)$ is implemented with bidirectional encoders such as BERT~\cite{devlin-etal-2019-bert}.
We provide the details of the MLP in Appendix \ref{sec:document-scorer} and the details of the embedding function below, as part of the sentence selection model description.

% \justin{move to merged section}
% Document embeddings $\text{emb}(d)$ are obtained by feeding the input 
% ``\texttt{[CLS]} $x$ \texttt{[SEP]} $d$'' to a bidirectional encoder,
% such as BERT~\cite{devlin-etal-2019-bert}, and taking the final state of the
% \texttt{[CLS]} token.
% %To obtain an embedding for a document, we feed ``\texttt{[CLS]} $x$ \texttt{[SEP]} $d$'' into the encoders and take the final state of the \texttt{[CLS]} token as the embedding.
% \justin{rest in appendix}
% We note that the encoders can only accept inputs shorter than a fixed length (e.g., 512 tokens).
% To address this limitation, we partition documents into slices of $m$ sentences and compute the embedding for each slice individually.
% We denote a slice for a document $d$ as $d^{i:j}$ that starts at the $i$th sentence and ends before the $j$th sentence.
% Let $i \in \text{range}(0, |d|, p)$, we approximate $\text{emb}(d)$ by the following aggregation,
% \begin{equation*}
%     \text{emb}(d) \approx \left\lfloor \frac{|d|}{m}\right\rfloor \sum_i \text{emb}(d^{i:i+p}).
% \end{equation*}

\paragraph{Sentence Set Selection}
%We now describe the parameterization for the rationale model, $p(\bm{z}_1, \bm{z}_2|d_1, d_2)=p(\bm{z}_1|d_1)p(\bm{z}_2|d_2)$.
%Because the interaction between documents has already been taken into account when choosing documents, we make a conditional independence assumption when choosing rationales: $\bm{z}_1$ and $\bm{z}_2$ are independent given their respective documents $d_1,d_2$.
% yielding $$p(\bm{z}_1, \bm{z}_2|d_1, d_2)=p(\bm{z}_1|d_1)p(\bm{z}_2|d_2).$$
%Therefore, $p(\bm{z}_1, \bm{z}_2|d_1, d_2)=p(\bm{z}_1|d_1)p(\bm{z}_2|d_2)$, and we describe a parameterization that is agnostic to selecting sentences from either $d_1$ or $d_2$. 
% We now describe the parameterization for the sentence selection model, $p(\bm{z}_i|d_i,x)$.
Within each document $d_i$, we select $\bm{z}_i \in \mathcal{P}(d_i)$, a power set of all sentences in $d_i$.
We rely on a sentence set scoring function $g(\bm{z}_i, x)$, similar to the document set scoring function,
which captures all relationships between selected sentences and the question.
The sentence set selection model is given by
\begin{equation*}
    p(\bm{z}_i\mid d_i, x) \propto \text{exp}(g(\bm{z}_i,x)),
\end{equation*}
which is globally normalized over all valid subsets of sentences in the document $d_i$.
% and the parameter $\bm{w}$ is a learned weight vector.

%We provide the details of the embedding function below.

%Let $\bm{w}$ be an $n$-dimensional learnable vector.
%Because there are exponentially many possible rationales, computing an embedding for every one of them is intractable.
%Instead, we compute an embedding for each sentence $s \in d$.
%To obtain the rationale embedding of a particular $\bm{z}$, we aggregate sentence embeddings $\text{emb}(s)$ for every sentence $s \in \bm{z}$ via mean.
%Here, we reuse the computation from the first stage where we encode documents.
%Specifically, instead of feeding ``[CLS] $x$ [SEP] $d$'' to an encoder, we modify it to be ``[CLS] $x$ [SEP] [UNK] $s_1$ [UNK] $s_2$ ... [UNK] $s_{|D|}$''.
%We take the last hidden state of each [UNK] token to be the embedding for the sentence following right after that [UNK] token.
%We thus encode documents and sentences at the same time.

% Because each rationale $z$ is a subset of sentences in $d$, there are exponentially many possible rationales, and therefore computing an embedding for each rationale separately is intractable.
% Instead, we compute an embedding for each sentence $s \in d$, then combine them according to the rationale $\bm{z}$.
% Specifically, instead encoding ``[CLS] $x$ [SEP] $d$'' directly, we insert [UNK] tokens in-between sentences:
% %We use the representations of [UNK] tokens as sentence representations in order to obtain rationale representations:
% \begin{align*}
%     u &= \texttt{[CLS]}x\texttt{[SEP]}\texttt{[UNK]}s_1\texttt{[UNK]}\ldots\\
%     \text{emb}(\bm{z})&= \sum_{j\in\mathcal{J}}\text{BERT}(u)_j,
% \end{align*}
% where $\mathcal{J}$ is the set of indices of \texttt{[UNK]} tokens that correspond to sentences in the rationale $s\in z$.
% This allows for contextual representations of sentences that depend on the whole document and also cheaply combine into rationale representations.

% Both the document and sentence selection models rely on contextual embeddings of the question $x$, document $d_i$, and sentence subsets $\bm{z}_i$ of $d_i$.
Computing $p(\bm{z}_i\mid d_i, x)$ requires enumerating all sentences subsets, which is intractable.
%To compute $g$, it is intractable to directly encode sentence subsets, as that would require running an encoder on exponentially many sequences.
% Rather than directly encoding subsets of documents and sentences,
We instead extend the approach of \citet{li2022easy}, which obtains document and contextual sentence representations in a single encoding step.
%We first interleave sentences with a special \texttt{[SPC]} token at known positions $k$:
We insert a special \texttt{[SPC]} token at the beginning of each sentence, shown here at positions $k_1, k_2, \dotsc$,
\begin{align*} u = \texttt{[C}&\texttt{LS]} \text{\{x\}} \texttt{[SEP]} &\texttt{[S}&\texttt{PC]}\ldots &\texttt{[S}&\texttt{PC]}\ldots. \\
    &0 && k_1 && k_2
\end{align*}
We then obtain sentence subset $\text{emb}(\bm{z}_i)$ embeddings by feeding this to an encoder-only model such as BERT~\cite{devlin-etal-2019-bert} and taking the average of the contextual embeddings of the special tokens corresponding to the sentences in $\bm{z}_i$:
\begin{align*}
    % \text{emb}(d_i)&= \text{encoder}(u)_0,\\
    \text{emb}(\bm{z}_i, x)&= \frac{1}{|\bm{z}_i|}\sum_{j \in \bm{z}_i}\text{encoder}(u)_{k_j}.
\end{align*}
Finally, let $v$ be a learnable vector, $g(\bm{z}_i, x) = v^T \text{emb}(\bm{z}_i, x)$
In practice, we note that encoder methods have a maximum input length, which can prevent full document encodings. We provide the details of long document encoding in Appendix~\ref{sec:encoding-long-docs}.
We also only consider subsets of up to a fixed max length.

%and obtaining the hidden states of the \texttt{[CLS]} and \texttt{[UNK]} tokens appearing before selected sentences respectively:
%This allows for contextual representations of sentences that depend on the whole document and also cheaply combine into rationale representations.

% We compute the embeddings for documents and sentence subsets by  $\text{emb}(\bm{z}_i)$ by first encoding the document $d_i$
% then combining only the representations of chosen sentences $\bm{z}_i$.
% We 
% \begin{align*}
%     u &= \texttt{[CLS]}x\texttt{[SEP]}\texttt{[UNK]}s_1\texttt{[UNK]}\ldots\\
%     \text{emb}(\bm{z})&= \sum_{j\in\mathcal{J}}\text{BERT}(u)_j,
% \end{align*}
% where $\mathcal{J}$ is the set of indices of \texttt{[UNK]} tokens that correspond to sentences in the rationale $s\in z$ \cite{cite}.
% This allows for contextual representations of sentences that depend on the whole document and also cheaply combine into rationale representations.

\paragraph{Answer Generation}
Parameterization of the answer generation model, $p(y\mid\bm{z}, x)$, is done using a sequence-to-sequence model where the question and rational are fed to an encoder, and that answer is generated. This process is complicated by the fact that answers can take on different forms, depending on specific QA tasks such as Boolean QA, multiple-choice QA, extractive QA, and abstractive QA, etc.
We can therefore use a sequence-to-sequence model such as BART~\cite{lewis-etal-2020-bart} and T5~\cite{2020t5}, and provide prompt templates for the different variants of the task, given in the next section.
% The exact parameterization of the answer model is task-dependent.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/explain.pdf}
%     \caption{An overview for the proposed approach, \eba, makes inference in three stages, in which it chooses documents, rationales, and answers sequentially.}
%     \label{fig:inference}
% \end{figure}

\subsection{Training and Inference}
To learn an explainable multi-hop QA system, \eba\ optimizes an approximation of the marginal likelihood. 
%$\mathcal{L}(\cdot)$, with respect to parameters $\theta$ (the encoder embeddings and sequence-to-sequence model) over training examples:
The marginal likelihood,
\begin{equation*}
    \mathcal{L(\theta)} = \text{log} \sum_{\bm{d}, \bm{z}} p_\theta(y, \bm{z}, \bm{d}\mid x),
\end{equation*}
is intractable, as it requires computing $p(y\mid\bm{z},x)$ under the answer generation model
for every valid set of sentences across documents.
We instead optimize a top-K Viterbi approximation of the marginal likelihood.
Given
\begin{align*}
    \mathcal{S}_{}^k &= \argtopk_{\bm{d}} p_\theta(\bm{d}\mid x)\\
    \mathcal{S}^k_{\bm{d}} &= \argtopk_{\bm{z}}
        %p_\theta(\bm{z}|\bm{d},x).
        %p(\bm{z}_i \mid d_i,x).
        \prod_i p_\theta(\bm{z}_i \mid d_i,x),
\end{align*}
we use the following approximation of the marginal likelihood
as our training objective:
\begin{equation*}
    \mathcal{L(\theta)} \approx \text{log} \sum_{\bm{d}\in \mathcal{S}^k} \sum_{\bm{z}\in \mathcal{S}^k_{d}} p_\theta(y, \bm{z}, \bm{d}\mid x).
\end{equation*}
%This approximate objective takes $O(k^2 + |\bm{d}|^2)$ computation.
%We summarize how \eba \ performs inference in three stages in Figure~\ref{fig:inference}.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/explain.pdf}
%     \caption{At test time, \eba \ first selects the best document set according to probabilities; \eba \ then selects the best sentence subset for each document in the best document set. Finally, \eba \ combines the best sentence subsets to generate an answer.
%     }
%     \label{fig:prediction}
% \end{figure}

At test time, we must choose the best documents and rationales.
Similar to training, we first choose the most likely pair of documents from $S^1$, then the most likely rationale from $S_{\bm{d}}^1$.
%We illustrate this process in Figure \ref{fig:prediction}.
%First, we choose a pair of documents by
%\begin{equation*}
%    d_1, d_2 = \argmaxB_{D_1, D_2} P_\theta(D_1, D_2).
%\end{equation*}
%Then, we choose a rationale by
%\begin{equation*}
%    \bm{z}=\argmaxB_{\bm{Z}_1, \bm{Z}_2} %P_\theta(\bm{Z}_1|D_1=d_1) P_\theta(\bm{Z}_2|D_2=d_2).
%\end{equation*}
Finally, for span-based QA, we generate an answer by performing greedy search on the answer generation model $p(y|\bm{z},x)$; for Boolean QA or multiple-choice QA, we normalize the answers between different choices and take $\argmaxB_{y}p(y|\bm{z},x)$.

%\paragraph{Reasoning over a Single Document.}
%In the case of $|\bm{D}|=1$, we can omit the document model.
%Let $\mathcal{S} = \argtopk_{\bm{Z}} P_\theta(\bm{Z}|X)$, the objective $\mathcal{L}(\cdot)$ thus becomes,
%\begin{equation*}
%    \mathcal{L(\theta)} \approx \text{log} \sum_{z\in \mathcal{S}} P_\theta(Y, \bm{Z}|X).
%\end{equation*}
%At test time, \eba \ chooses the rationale by
%\begin{equation*}
%    \bm{z}=\argmaxB_{\bm{Z}} P_\theta(\bm{Z}|X).
%\end{equation*}
%Finally, how to choose answers remains the same.

==> exNLP_acl2023 (Copy)/old_method.tex <==
\section{Method}
% \label{fig:generative}
% \end{figure}
% \begin{figure}[t]
%   \begin{center}
%   \scalebox{.85}{
%     \begin{tikzpicture}
%     \node[latent] (d) {$D_i$};
%     \factor[left=of d, xshift=-0.2cm] {dp} {} {} {} ;
%     \node[latent, right=of d] (z) {$Z_i^j$};
%     \factor[left=of z, xshift=-0.1cm] {zp} {} {} {} ;
%     \node[obs, right=of z] (y) {$Y$};
%     \factor[left=of y, xshift=-0.1cm] {yp} {} {} {} ;
%     \edge {dp} {d};
%     \edge {d} {z};
%     \edge {z} {y};
%     \plate [inner sep=.23cm,xshift=-.1cm,yshift=.2cm] {plate2} {(z)} {$J$};
%     \plate [inner sep=0.25cm,xshift=-.15cm,yshift=.2cm] {plate1} {(plate2)(d)} {$I$};
%     \end{tikzpicture}
%     }
%   \end{center}
% \caption{The graphical model for the generative process for multi-hop QA when $m=2$. Because every other random variable depends on $X$, we omit it for the sake of simplicity.}
% \label{fig:generative}
% \end{figure}

% \begin{figure}[!t]
%     \textbf{\textit{{\small Parallel Reasoning:}}}\\
%     \framebox{
%     \parbox{0.45\textwidth}{
%     \small
%     \textbf{Q:} Are Hattiesburg–Laurel Regional Airport and Wilmington International Airport both located in North Carolina? \noindent \smallskip \newline
%     \textbf{Document A, Wilmington International Airport:} \newline
%     Wilmington International Airport is a public airport located just north of Wilmington, North Carolina. [$\dotsc$]\newline
%     \textbf{Document B, Hattiesburg–Laurel Regional Airport:} \newline
%     Hattiesburg–Laurel Regional Airport, also Airport City, is a public airport in Jones County, Mississippi. [$\dotsc$]\smallskip \newline
%     \textbf{A:} No}
%     }\vspace*{2pt}
%     \textbf{\textit{{\small Sequential Reasoning:}}}\\
%     \framebox{
%     \parbox{0.45\textwidth}{
%     \small
%     \textbf{Q:} Which team does the player named 2015 Diamond Head Classic’s MVP play for? \noindent \smallskip \newline
%     \textbf{Document A, 2015 Diamond Head Classic:} \newline
%     [$\dotsc$] Buddy Hield was named the tournament’s MVP.\newline
%     \textbf{Document B, Buddy Hield:} \newline
%     Buddy Hield is a Bahamian professional basketball player for the Sacramento Kings of the NBA. [$\dotsc$]\smallskip \newline
%     \textbf{A:} Sacramento Kings}
%     }
%     \caption{Demonstrations on when parallel and sequential reasoning are applied in multi-hop reasoning. Irrelevant sentences are removed from the documents.} \label{fig:example}
% \end{figure}
% \begin{figure}[t]
%   \begin{center}
%   \scalebox{.85}{
%     \begin{tikzpicture}
%     \node[obs] (x) {$X$};
%     \node[latent, right=of x] (z) {$Z$};
%     \node[obs, right=of z] (y) {$Y$};
%     \edge {x} {z};
%     \edge {z} {y};
%     \draw[->] (x) to[bend left] (y);
%     \end{tikzpicture}
%     }
%   \end{center}
% \caption{The graphical model for the generative process for multi-hop QA when $|\bm{D}|=1$.}
% \label{fig:generative}
% \end{figure}
% We now describe \eba, an explainable approach for multi-hop QA that requires no rationale supervision.


\begin{figure}
    \centering
    \small
    \framebox{
    \parbox{0.45\textwidth}{
    \small
    \textbf{Q:} A medieval fortress in Dirleton, East Lothian, Scotland borders on the south side of what coastal area? \noindent \smallskip \newline
    \textbf{Document A, Yellowcraig:} \newline
    \support{Yellowcraig, less commonly known as Broad Sands Bay, is a coastal area of forest, beach and grassland in East Lothian, south-east Scotland.} Yellowcraig is partly within the Firth of Forth Site of Special Scientific Interest (SSSI). \support{It is bordered to the north by the Firth of Forth, to the south by the village of Dirleton and Dirleton Castle, to the east by the North Berwick West Links golf course, and to the west by the Archerfield Estate and Links golf courses.}\newline
    \textbf{Document B, Dirleton Castle:} \newline
    \support{Dirleton Castle is a medieval fortress in the village of Dirleton, East Lothian, Scotland.} It lies around 2 mi west of North Berwick, and around 19 mi east of Edinburgh. The oldest parts of the castle date to the 13th century, and it was abandoned by the end of the 17th century.\smallskip \newline
    \textbf{A:} Yellowcraig}
    }
    \caption{A multi-hop QA example. The sentences used to derive the answer are highlighted in \support{blue italics}.}
    \label{fig:multihop_example}
\end{figure}
Figure~\ref{fig:multihop_example} shows a multi-hop QA example, which starts with a question, accompanied by one or multiple supporting documents, and an answer can be derived from a set of sentences in the documents.

We start with multi-hop reasoning over a single document.
Then, we show by adding a document selection module, \eba \ can easily be extended to reason over multiple documents.
Formally, a multi-hop QA example consists of a question $X$, a document $D$, and an answer $Y$.
An explainable method for multi-hop QA not only predicts $Y$, but also generates a rationale $Z \in \mathcal{P}(D)$, which is a minimal set of sentences in $D$ from which $Y$ can be derived.
Hops are defined at the sentence level; if a question requires reasoning over multiple sentences to reach the answer, then we consider it to be a multi-hop QA problem.

The goal of multi-hop QA is to produce a probability distribution over answers $Y$ to questions $X$, defined by $P(Y|X)$.
In order to produce answers $Y$, \eba \ first identifies unobserved rationales $Z$ given question $X$, then chooses answers $Y$ given both $X$ and $Z$.
This yields the joint distribution
\begin{align*}
    P(Y,Z|X) = P(Z|X)P(Y|X,Z).
\end{align*}
%illustrated in Figure \ref{fig:generative}

% The goal of multi-hop QA is to produce a probability distribution over answers $Y$, defined by $P(Y|X)$.
% \eba \ assumes a data generating process shown in Figure~\ref{fig:generative}, where rationales $Z$ are unobserved but directly affect $Y$.
% According this generative process, \eba \ proceeds in two stages:
% \begin{align*}
%     P(Y,Z|X) = P(Z|X)P(Y|X,Z)
% \end{align*}
This factorization naturally provides explainability -- in the first phase, \eba \ identifies rationales $Z$ based on the information contained in $X$; in the second phase, \eba \ derives answers $Y$ from both questions $X$ and rationales $Z$.
Our goal is to train \eba \ to produce high $P(Y|X,Z)$ for correct rationales and low $P(Y|X,Z)$ for incorrect rationales.
% Formally, a multi-hop QA example consists of a question $X$, a set of documents $\bm{D}$, and an answer $Y$.
% We assume that each task pre-specifies the number of relevant documents to be $m$.
% An explainable method not only predicts $Y$, but also generates a rationale $Z \in \mathcal{P}(\bm{D})$, which is a minimal set of sentences in the $m$ documents from which $Y$ can be derived.
% We first describe \eba \ for $|\bm{D}|=1$, where there is no need for document selection.
% We then show and generalize it to reasoning over multiple documents.

% Here, we consider exactly two documents are relevant to the question, but \eba \ can be easily extended to more documents.
% We assume there are unobserved variables $D_1$ and $D_2$, representing two supporting documents.
% Further, there are another two unobserved variables $Z_1$ and $Z_2$, representing sets of sentences selected from $D_1$ and $D_2$, respectively.
% We specify the generative process for multi-hop QA in Figure~\ref{fig:generative}, where only question $X$ and answer $Y$ are observed.
% Because all the remaining variables condition on $X$, we omit it from the graphical model.

% Without document selection, the generative model proceeds in two phases.
% At the first phase, the model selects documents, which naturally leads to a model design choice -- whether to make an independence assumption between the two documents.
% With the independence assumption, each document can be considered individually; therefore, selecting documents has a low complexity that is linear to the number of documents.
% To illustrate how our design choice is made, we first differentiate two types of multi-hop reasoning in Figure~\ref{fig:example}.
% To answer the first question, it is possible to independently identify what documents may be needed to derive an answer.
% Thus, selecting each of the two documents can be done in parallel.
% However, in the second question, it is not possible to identify Document B without knowing the information in Document A.
% Thus, answering the second question requires reasoning about the two documents in a specific order.
% To capture this sequential nature of multi-hop reasoning, we condition $D_2$ on both $X$ and $D_1$, so that \eba \ has enough expressive power to answer the questions that requires performing sequential reasoning.

% At the second stage, the model chooses a set of sentences from the documents.
% Because we already take into account the relation between multiple documents at the first stage, $Z_2$ is made independent of $Z_1$.
% We further point out that the number of choices of $Z_1$ and $Z_2$ are exponential to the number of sentences in $D_1$ and $D_2$, respectively.
% For this reason, approximating distributions over $Z_1$ and $Z_2$ separately has a lower complexity than approximating a distribution over $Z_1 \times Z_2$.
% Finally, answer $Y$ is predicted with both $Z_1$ and $Z_2$.
% In summary, our probabilistic model places a distribution over $(D_1, D_2, Z_1, Z_2, Y)$ and factorizes according to the three phases as follows:
% \begin{align*}
%     P(D_1, D_2, Z_1, Z_2, Y) = &P(D_1)P(D_2|D_1) \\
%     \cdot &P(Z_1|D_1)P(Z_2|D_2) \\
%     \cdot &P(Y|Z_1, Z_2)
% \end{align*}

\subsection{Parameterization}
We now turn to how \eba \ parameterizes each model.
We first describe the parameterization for the rationale model $P(Z|X)$.
Let $\text{emb}: \mathcal{V}^* \rightarrow \mathbb{R}^n$ be an embedding function that maps a sequence of text $\mathcal{V}^*$ to a real-valued vector of $n$ dimensions, where $\mathcal{V}$ is a vocabulary.
%Let $W: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a linear layer,
Let $\bm{w}$ be an $n$-dimensional vector,
\begin{equation*}
    %P(Z=z|X) = \frac{e^{W(\text{emb}(z))}}{\sum_{z'} e^{W(\text{emb}(z'))}}.
    P(Z=z|X=x) \propto \text{exp}(\langle \bm{w}, \text{emb}(z, x)\rangle)
\end{equation*}
Because there are exponentially many possible rationales, computing an embedding for every one of them is intractable.
Instead, we compute an embedding for each sentence $s \in D$.
To obtain the rationale embedding of a particular $z$, we aggregate sentence embeddings $\text{emb}(s)$ for every sentence $s \in z$ via mean.
In practice, $\text{emb}(\cdot)$ is implemented with bidirectional encoders such as BERT~\cite{devlin-etal-2019-bert}.
The input we feed to the encoders is $D$, with an [UNK] token inserted before each sentence: ``$X$ [SEP] [UNK] $s_1$ [UNK] $s_2$ ... [UNK] $s_{|D|}$''.
We take the last hidden state of each [UNK] token to be the embedding for the sentence following right after that [UNK] token.
Therefore, computing $P(Z|X)$ only requires one forward pass of the encoders.
To summarize, compared to \citet{atanasova2022diagnostics} where all sentences in a rationale are all predicted in a fully independent way, we are able to add dependency between sentences with little overhead via a parameterization trick.

\begin{table}[t]
\centering
\small
\begin{tabular}{p{0.07\linewidth} p{0.04\linewidth} p{0.75\linewidth}}
\toprule
& \cellcolor{blue!15} In          & \cellcolor{blue!15} {\noindent \color{red} \textit{A claim to be verified is that}} $X$ {\noindent \color{red} \textit{We have following facts:}} $Z$ \\
      & \cellcolor{blue!15} Out                        & \cellcolor{blue!15} {\noindent \color{red} \textit{The claim is thus}} \{supported/refuted\}. \\
BQA  & \cellcolor{green!15} In          & \cellcolor{green!15} {\noindent \color{red} \textit{A claim to be verified is that}} Steve Wozniak designed homes. {\noindent \color{red} \textit{We have following facts:}} Steve Wozniak primarily designed the 1977 Apple II , known as one of the first highly successful mass-produced microcomputers. \\

     & \cellcolor{green!15} Out                        & \cellcolor{green!15} {\noindent \color{red} \textit{The claim is thus}} refuted. \\ \midrule

& \cellcolor{blue!15} In         & \cellcolor{blue!15} {\noindent \color{red} \textit{Question:}} $X$ [SEP] $Z$ \\
           & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} {\noindent \color{red} \textit{Answer:}} $Y_1$ (\{correct/wrong\}) [SEP] {\noindent \color{red} \textit{Answer:}} $Y_2$ (\{correct/wrong\}) [SEP] ...  \\
MCQ & \cellcolor{green!15} In         & \cellcolor{green!15} {\noindent \color{red} \textit{Question:}} Name few objects said to be in or on Allan 's desk. [SEP] Opening a side drawer, he took out a piece of paper and his inkpot. \\
           & \cellcolor{green!15} Out                  & \cellcolor{green!15}  {\noindent \color{red} \textit{Answer:}} Eraser  (wrong) [SEP] {\noindent \color{red} \textit{Answer:}} Inkpot (correct) [SEP] {\noindent \color{red} \textit{Answer:}} Pen (correct) \\ \midrule

 & \cellcolor{blue!15} In         & \cellcolor{blue!15} $X$ [SEP] $Z$ \\
           & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} $Y$ \\
EQA & \cellcolor{green!15} In         & \cellcolor{green!15} Which American railroad, located in Southwestern Montana and Idaho, was backed by the Northern Pacific Railway? [SEP] The Gilmore and Pittsburgh Railroad (G\&P), now defunct, was an American railroad located in southwestern Montana and east-central Idaho. \\
           & \cellcolor{green!15} Out                  & \cellcolor{green!15} Gilmore and Pittsburgh Railroad \\
\bottomrule
\end{tabular}%
\caption{Example conversions from QA examples to text-to-text examples for Boolean QA (BQA), multiple-choice QA (MCQ), and extractive QA (EQA). Templates are in purple cells, followed by specific examples in green cells. Template keywords are highlighted in {\color{red} \textit{red italics}}.}
\label{tab:conversion}
\end{table}

We then describe the parameterization for the answer model $P(Y|X, Z)$.
Because \citet{khashabi-etal-2020-unifiedqa} show that text-to-text models can handle QA tasks of all formats, they become a natural choice for parameterizing $P(Y|Z_1, Z_2)$.
Examples of such models are BART~\cite{lewis-etal-2020-bart} and T5~\cite{2020t5}.
The exact parameterization of the answer model is task-dependent.
In Table~\ref{tab:conversion}, we demonstrate how to convert QA examples of different forms to text-to-text examples.
For Boolean QA, we take the problem of fact checking as an example, in which a claim $X$ needs to be classified as whether it is supported (0) or refuted (1) with the accompanying documents $\bm{D}$.
Inspired by prompting~\cite{brown2020language}, instead of directly inputting $X, Z$ and outputting $0/1$, we connect them with instructional prompts.
For multiple-choice QA, we consider a general case where there is a varying number of choices per example, and an unknown number of the choices is correct.
We note that determining the truth value of one answer choice may not require all sentences in the rationale; therefore, knowing the truth value of one answer choice does not have enough information to inform the entire rationale.
For this reason, we stack all answer choices attached with their truth values as outputs to supervise the model.
Finally, extractive QA can naturally be formulated as a text-to-text problem, where the input is $X$ [SEP] $Z$, and the output is $Y$.

\subsection{Training \& Inference}
To learn an explainable multi-hop QA system, \eba \ maximizes the likelihood function $\mathcal{L}(\cdot)$ with respect to parameters $\theta$ for all training examples:
\begin{equation*}
    \mathcal{L(\theta)} = \text{log} \sum_{Z} P_\theta(Z|X) P_\theta(Y|X, Z).
\end{equation*}
We note that even though $P_\theta(Z|X)$ can be computed efficiently with our parameterization trick, $P_\theta(Y|X, Z)$ requires encoder-decoder models to perform $|Z|$ forward passes.
Thus, the exact computation of $\mathcal{L(\theta)}$ will still be intractable when the number of sentences in $D$ is large.
We thus approximate this objective by
\begin{equation*}
    \mathcal{L(\theta)} \approx \text{log} \sum_{z\in \mathcal{S}} P_\theta(Z|X) P_\theta(Y|X, Z),
\end{equation*}
where $\mathcal{S} = \argtopk_{Z} P_\theta(Z|X)$.
At test time, \eba \ chooses the rationale by
\begin{equation*}
    z=\argmaxB_{Z} P_\theta(Z|X).
\end{equation*}
Therefore, rationales are selected by conditioning only on the questions without peeking at the answers.
Finally, when predicting the answer, we generate an answer by performing greedy search on $P(Y|Z=z, X)$ for span-based QA.
For Boolean QA or multiple-choice QA, we normalize over different answer choices and take the answer to be $\argmaxB_{Y}P(Y|Z=z, X)$.

\begin{figure}[t]
  \begin{center}
  \scalebox{.85}{
    \begin{tikzpicture}
    \node[obs] (x) {$X$};
    \node[latent, right=of x] (d) {$D_1$};
    \node[latent, below=of d] (dd) {$D_2$};
    \node[latent, right=of d] (z) {$Z_1$};
    \node[latent, right=of dd] (zz) {$Z_2$};
    \node[obs, right=of z] (y) {$Y$};
    \edge {x} {d};
    \edge {x} {dd};
    \draw[->] (x) to[bend left] (z);
    \draw[->] (x) to[bend left] (y);
    \edge {x} {zz};
    \edge {d} {dd};
    \edge {d} {z};
    \edge {dd} {zz};
    \edge {z} {y};
    \edge {zz} {y};
    \end{tikzpicture}
    }
  \end{center}
\caption{The graphical model is updated to handle multi-hop QA for $m=2$.}
\label{fig:generative2}
\end{figure}
\subsection{Reasoning over Multiple Documents}
Resolving queries may often involve reasoning over large contexts involving multiple documents. We extend \eba \ to handle multiple documents by making two modifications to the previous setup: single documents $D$ become a set of documents $\bm{D}$, and not every document in $\bm{D}$ is relevant to the question.
We assume the number of relevant documents $m$ is pre-specified by each task.
Here, we describe how to extend \eba \ to $m=2$.
We let $D_1$ and $D_2$ to be the first and the second relevant documents, respectively.
In a rationale $Z=(Z_1, Z_2)$, $Z_1 \subseteq D_1$ and $Z_1 \subseteq D_1$.
We update the graphical model in Figure~\ref{fig:generative2}.
With the new data generating process, \eba \ proceeds in three stages (with $X$ omitted for the sake of brevity),
\begin{align*}
    P(D_1, D_2, Z_1, Z_2, Y) = &P(D_1)P(D_2|D_1) \\
    \cdot &P(Z_1|D_1)P(Z_2|D_2) \\
    \cdot &P(Y|Z_1, Z_2).
\end{align*}
The only addition is \eba \ now starts with document selection.
After two documents are chosen, we repeat the procedure described in the previous section.
We note that, because we want to optimally trade off between accuracy and efficiency, we only consider the dependency between documents in the first stage and assume documents are independent from each other in the second stage.
We show that, with a few tweaks \eba \ can be extended to reason over multiple documents.

\paragraph{Parameterization for the Document Model $P(D_1, D_2|X)$.}
Let $f: D_1 \times D_2 \rightarrow \mathbb{R}$. We assume
\begin{equation*}
    P(D_1, D_2) \propto \exp(f(D_1, D_2)).
\end{equation*}
Because computing an embedding for every pair of documents take quadratic time, we combine two documents in the embedding space via Siamese networks~\cite{reimers-gurevych-2019-sentence}.
Let $\text{e}_{D_1}=\text{emb}(D_1)$ and $\text{e}_{D_2}=\text{emb}(D_2)$, and $[\cdot]$ be a concat operator:
\begin{equation*}
\text{emb}([D_1, D_2]) \approx [\text{e}_{D_1},\text{e}_{D_2},|\text{e}_{D_1}-\text{e}_{D_2}|].
\end{equation*}
Let $\text{MLP}: \mathbb{R}^{3n} \rightarrow \mathbb{R}$ be a multilayer perceptron,
\begin{equation*}
    f(D_1, D_2) = \text{MLP}(\text{emb}([D_1, D_2])).
\end{equation*}
Finally, $P(D_1, D_2|X)$ is normalized over document pairs.
Document embeddings can be obtained almost for free by reusing the computation in the rationale model, where we input the encoders with a document to get an embedding for every sentence.
We append a [CLS] token to the left of the original input and use the last hidden state of this token to be the document embedding.
We note that the encoders can only accept inputs shorter than a fixed length (e.g., 512 tokens).
To address this limitation, we partition documents into slices of $m$ sentences and compute the embbeding for each slice individually.
We denote a slice for a document $D$ as $D^{i:j}$ that starts at the $i$th sentence and ends before the $j$th sentence.
Let $i \in \text{range}(0, |D|, p)$, we approximate $\text{emb}(D)$ by the following aggregation,
\begin{equation*}
    \text{emb}(D) \approx \lfloor \frac{|D|}{m}\rfloor \sum_i \text{emb}(D^{i:i+p}).
\end{equation*}
\paragraph{Training \& Inference}
We describe approximation of the updated likelihood function.
Let $\mathcal{S}_d = \argtopk_{D_1,D_2} P_\theta(D_1, D_2)$.
Let $z_d=(z_1, z_2)$ be a rationale from a given pair of documents $d=(d_1, d_2)$, and $\mathcal{S}_{z, d} = \argtopk_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2)$.
Then,
\begin{equation*}
    \mathcal{L(\theta)} \approx \text{log} \sum_{d\in \mathcal{S}_d} \sum_{z_d\in \mathcal{S}_{z, d}} P_\theta(Y, Z_1, Z_2, D_1, D_2).
\end{equation*}
%\justin{important to emphasize not using posterior}
At test time, we choose a pair of documents by
\begin{equation*}
    d_1, d_2 = \argmaxB_{D_1, D_2} P_\theta(D_1, D_2).
\end{equation*}
Then, we choose a rationale by
\begin{equation*}
    z=\argmaxB_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2).
\end{equation*}
Finally, predicting answers remains unchanged.
% We first consider parametering the document models.
% %Because $P(D_1)P(D_2|D_1)=P(D_2)P(D_1|D_2)$, to avoid symmetric document pairs, instead of identifying the two documents in a sequential manner, we assume
% Let $f: D_1 \times D_2 \rightarrow \mathbb{R}$. We assume
% \begin{equation*}
%     P(D_1, D_2) \propto e^{f(D_1, D_2)}.
% \end{equation*}
% Let $\text{emb}: \bm{T} \rightarrow \mathbb{R}^n$ be an embedding function that maps a text sequence $\bm{T}$ to a real-valued vector of $n$ dimensions.
% Because computing the exact embedding for every pair of documents is computationally expensive, we combine two documents in the embedding space via Siamese networks~\cite{reimers-gurevych-2019-sentence}.
% Let $\text{e}_{D_1}=\text{emb}(D_1)$ and $\text{e}_{D_2}=\text{emb}(D_2)$, and $[\cdot]$ be a concat operator:
% \begin{equation*}
% \text{emb}([D_1, D_2]) \approx [\text{e}_{D_1},\text{e}_{D_2},|\text{e}_{D_1}-\text{e}_{D_2}|].
% \end{equation*}
% Let $\text{MLP}: \mathbb{R}^{3n} \rightarrow \mathbb{R}$ be a multilayer perceptron,
% \begin{equation*}
%     f(D_1, D_2) = \text{MLP}(\text{emb}([D_1, D_2])).
% \end{equation*}
% Finally, $P(D_1, D_2)$ is normalized over document pairs.
% In practice, $\text{emb}(\cdot)$ is implemented with bidirectional encoders such as BERT~\cite{devlin-etal-2019-bert}.
% To obtain an embedding for a document, we feed ``[CLS] $X$ [SEP] $D$'' into the encoders and take the final state of the [CLS] token as the embedding.
% We note that the encoders can only accept inputs shorter than a fixed length (e.g., 512 tokens).
% To address this limitation, we partition documents into slices of $m$ sentences and compute the embbeding for each slice individually.
% We denote a slice for a document $D$ as $D^{i:j}$ that starts at the $i$th sentence and ends before the $j$th sentence.
% Let $i \in \text{range}(0, |D|, p)$, we approximate $\text{emb}(D)$ by the following aggregation,
% \begin{equation*}
%     \text{emb}(D) \approx \lfloor \frac{|D|}{m}\rfloor \sum_i \text{emb}(D^{i:i+p}).
% \end{equation*}

% We then turn to parameterization of the rationale models.
% Since we let $P(Z_1|D_1)$ and $P(Z_2|D_2)$ share the same parameterization, we describe a general model $P(Z|D)$.
% $Z$ consists of all sentence combinations in $D$.
% %Let $\text{emb}_Z: Z \rightarrow \mathbb{R}^n$ and $W: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a linear layer,
% Let $W: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a linear layer,
% \begin{equation*}
%     P(Z=z|D) = \frac{e^{W(\text{emb}(z))}}{\sum_{z'} e^{W(\text{emb}(z'))}}.
% \end{equation*}
% %$\text{emb}_Z(\cdot)$ is also implemented with bidirectional encoders.
% For efficiency, we reuse the computation from the document models.
% Specifically, instead of feeding ``[CLS] $X$ [SEP] $D$'' to an encoder, we modify it to be ``[CLS] $X$ [SEP] [UNK] $D^1$ [UNK] $D^2$ ... [UNK] $D^{|D|}$''.
% That is, we insert a [UNK] token before each sentence and take the last hidden state of the token as the sentence embedding.
% Again, computing the exact embedding for every rationale $z$ is intractable.
% Options for approximating the embedding for $z$ are to combine individual sentence embeddings by max-pooling, sum, and mean.
% We choose to use mean, but they all lead to similar performance.

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{p{0.07\linewidth} p{0.04\linewidth} p{0.75\linewidth}}
% \toprule
% & \cellcolor{blue!15} In          & \cellcolor{blue!15} {\noindent \color{red} \textit{A claim to be verified is that}} $X$ {\noindent \color{red} \textit{We have following facts:}} $Z$ \\
%       & \cellcolor{blue!15} Out                        & \cellcolor{blue!15} {\noindent \color{red} \textit{The claim is thus}} \{supported/refuted\}. \\
% BQA  & \cellcolor{green!15} In          & \cellcolor{green!15} {\noindent \color{red} \textit{A claim to be verified is that}} Steve Wozniak designed homes. {\noindent \color{red} \textit{We have following facts:}} Steve Wozniak primarily designed the 1977 Apple II , known as one of the first highly successful mass-produced microcomputers. \\

%      & \cellcolor{green!15} Out                        & \cellcolor{green!15} {\noindent \color{red} \textit{The claim is thus}} refuted. \\ \midrule

% & \cellcolor{blue!15} In         & \cellcolor{blue!15} {\noindent \color{red} \textit{Question:}} $X$ [SEP] $Z$ \\
%            & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} {\noindent \color{red} \textit{Answer:}} $Y_1$ (\{correct/wrong\}) [SEP] {\noindent \color{red} \textit{Answer:}} $Y_2$ (\{correct/wrong\}) [SEP] ...  \\
% MCQ & \cellcolor{green!15} In         & \cellcolor{green!15} {\noindent \color{red} \textit{Question:}} Name few objects said to be in or on Allan 's desk. [SEP] Opening a side drawer, he took out a piece of paper and his inkpot. \\
%            & \cellcolor{green!15} Out                  & \cellcolor{green!15}  {\noindent \color{red} \textit{Answer:}} Eraser  (wrong) [SEP] {\noindent \color{red} \textit{Answer:}} Inkpot (correct) [SEP] {\noindent \color{red} \textit{Answer:}} Pen (correct) \\ \midrule

%  & \cellcolor{blue!15} In         & \cellcolor{blue!15} $X$ [SEP] $Z$ \\
%            & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} $Y$ \\
% EQA & \cellcolor{green!15} In         & \cellcolor{green!15} Which American railroad, located in Southwestern Montana and Idaho, was backed by the Northern Pacific Railway? [SEP] The Gilmore and Pittsburgh Railroad (G\&P), now defunct, was an American railroad located in southwestern Montana and east-central Idaho. \\
%            & \cellcolor{green!15} Out                  & \cellcolor{green!15} Gilmore and Pittsburgh Railroad \\
% \bottomrule
% \end{tabular}%
% \caption{Example conversions from QA examples to text-to-text examples for Boolean QA (BQA), multiple-choice QA (MCQ), and extractive QA (EQA). Templates are in purple cells, followed by specific examples in green cells. Template keywords are highlighted in {\color{red} \textit{red italics}}.}
% \label{tab:conversion}
% \end{table}

% Last but not least, because \citet{khashabi-etal-2020-unifiedqa} show that text-to-text models can handle QA tasks of all formats, they become a natural choice for parameterizing $P(Y|Z_1, Z_2)$.
% Examples of such models are BART~\cite{lewis-etal-2020-bart} and T5~\cite{2020t5}.
% The exact parameterization of the answer model is task-dependent.
% In Table~\ref{tab:conversion}, we demonstrate how to convert QA examples of different forms to text-to-text examples.
% %It is worth noting that we have gold labels to supervise the answer model.
% For Boolean QA, we take the problem of fact checking as an example, in which a claim $X$ needs to be classified as whether it is supported (0) or refuted (1) with the accompanying documents $\bm{D}$.
% Inspired by prompting~\cite{brown2020language}, instead of directly inputting $X, Z$ and outputting $0/1$, we connect them with instructional prompts.
% % The input to the seq2seq model is ``A claim to be investigated is that $X$ [SEP] We have following facts: $Z_1$ $Z_2$''.
% %$P(Y|Z_1, Z_2)$ is then normalized between two outputs: ``The claim is thus supported'' or ``The claim is thus refuted''.
% For multiple-choice QA, we consider a general case where there is a varying number of choices per example, and an unknown number of the choices is correct.
% We note that determining the truth value of one answer choice may not require all sentences in the rationale; therefore, knowing the truth value of one answer choice does not have enough information to inform the entire rationale.
% For this reason, we stack all answer choices attached with their truth values as outputs to supervise the model.
% % The input to the seq2seq model is ``Question: $X$ [SEP] $Z_1$ $Z_2$''.
% % The output to be generated is ``Answer: {Choice A} {correct/wrong} [SEP] ... [SEP] Answer: {Choice N} {correct/wrong}''.
% % Each choice bracket is filled by the answer choice text.
% Finally, extractive QA can naturally be formulated as a text-to-text problem, where the input is $X$ [SEP] $Z$, and the output is $Y$.

% \subsection{Training \& Inference}
% To learn an explainable multi-hop QA system, \eba \ maximizes the likelihood function $\mathcal{L}(\cdot)$ with respect to parameters $\theta$ for all training examples:
% \begin{equation*}
%     \mathcal{L(\theta)} = \text{log} \sum_{D_1, D_2, Z_1, Z_2} P_\theta(Y, Z_1, Z_2, D_1, D_2).
% \end{equation*}
% However, when the number of documents is large or when the documents have many sentences, computing $\mathcal{L}(\theta)$ becomes intractable.
% We thus describe an approximation to this objective.
% Let $\mathcal{S}_d = \argtopk_{D_1,D_2} P_\theta(D_1, D_2)$.
% Let $z_d=(z_1, z_2)$ be a rationale from a given pair of documents $d=(d_1, d_2)$, and $\mathcal{S}_{z, d} = \argtopk_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2)$.
% Then,
% \begin{equation*}
%     \mathcal{L(\theta)} \approx \text{log} \sum_{d\in \mathcal{S}_d} \sum_{z_d\in \mathcal{S}_{z, d}} P_\theta(Y, Z_1, Z_2, D_1, D_2).
% \end{equation*}
% At test time, we choose a pair of documents by
% \begin{equation*}
%     d_1, d_2 = \argmaxB_{D_1, D_2} P_\theta(D_1, D_2).
% \end{equation*}
% Then, we choose a rationale by
% \begin{equation*}
%     z=\argmaxB_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2).
% \end{equation*}
% Finally, for span-based QA, we generate an answer by performing greedy search on $P(Y|Z_1,Z_2=z)$; for Boolean QA or multiple-choice QA, we normalize the answers between different choices and take $\argmaxB_{Y}P(Y|Z_1,Z_2=z)$.

==> exNLP_acl2023 (Copy)/related.tex <==
\section{Related Work}
\paragraph{Explainable methods for multi-hop QA.}
Active research has been devoted to collecting human rationales for a wide range of QA tasks; a recent survey has identified 65 datasets that provide explanation annotations~\cite{wiegreffe2021teach}.
The appearance of such datasets has enabled rapid progress in supervised methods for extracting reasoning chains; we refer readers to~\citet{thayaparan2020survey} for a comprehensive survey.
While these supervised methods such as \citet{qi-etal-2019-answering} have achieved tremendous success on retrieving rationales, even in the open-domain setting~\footnote{While we only consider the distractor QA setting in this work, \eba \ can be combined with a rule-based retrieval system such as BM25 to be adapted to the open-domain setting.}, they can only be applied when rationale annotations are available.
However, such annotations do not always exist -- \citet{welbl-etal-2018-constructing} and \citet{yu2022crepe} propose two complex reasoning datasets that do not have rationale annotations.
In these cases, we need unsupervised rationale selection methods to still build explainable QA systems.

%Compared to fully supervised methods which require both answer and rationale annotations, methods that only assume access to answer annotations remain understudied.

%To reiterate, the task of interest is to predict answers for QA problems along with the rationales that lead to the answers.
%Note that we will refer to methods that only use answer supervision but not rationale supervision as \emph{unsupervised} methods.

Other works have explored multi-hop QA with only answer supervision but not rationale supervision. As in our work, Retrieve and Generate (\textsc{RAG}) \cite{NEURIPS2020_6b493230}, treats the rationale as a latent variable;
however, in \textsc{RAG} the open retrieval-stage is to find a single document, ignoring the connections between different documents. \textsc{RAG} also does not produce sentence-level rationales. Other works consider sentence rationales:
\citet{glockner-etal-2020-think} compute a score for every sentence pair and pick the sentence pair that has the highest score as the rationale for answer prediction, and
\citet{atanasova2022diagnostics} perform binary classification on whether individual sentences are included in the rationale with added constraints such as consistency and faithfulness.
The shared limitation of these methods is that they do not capture the dependency between more than two pieces of information.
\eba \ overcomes this limitation by performing multi-hop reasoning as document set prediction and sentence set prediction.

%The closest related work is~\citet{glockner-etal-2020-think}, which trains an explainable model by computing a cross entropy loss for every sentence pair to classify the answer and weighting the loss terms based on the classification confidence.
%At test time, they pick the sentence pair that has the highest confidence.
%Because they only consider at most two sentences, their method fails to capture the complex relation between different pieces of information across more than two sentences and across documents.

%\citet{atanasova2022diagnostics} identify several properties of rationales and develop loss functions to enforce the selected sentences to have such properties.
%Because their method does binary classification on whether each sentence is included in the rationale individually, it fails to capture dependencies between sentences.
% Because their method classifies each sentence individually, it would fail to identify all sentences in a rationale if the sentences need to be connected via bridges.

% Closely related is Retrieve and Generate (\textsc{RAG}) \cite{NEURIPS2020_6b493230}, which also treats the rationale as a latent variable.
% \textsc{RAG} models rationales as single documents, which fails to capture the dependency between documents and also does not produce sentence-level rationales.

%Additionally, when the number of rationales becomes large, the method is intractable; their experimental evaluation only considers rationales with up to two sentences.
Outside of unsupervised methods,
\citet{chen2019multi} propose a semi-supervised method which collects silver rationale annotations.
%Their silver rationales are paths from questions to answers, and the intermediate nodes are sentences.
%Two nodes are connected if they share a entity.
However, their method is limited to bridge-based questions, which is only one form of multi-hop reasoning; the other types can be found in \citet{trivedi2021musique}.
%other reasoning types include going from the general to the specific (e.g., ``fruits are healthy to eat'' -> ``apples are healthy to eat'').
\vspace*{-5pt}
\paragraph{Rationales as latent variables.}
%Outside of multi-hop QA, modeling rationales as latent variables has been extensively studied.
A focus for rationale methods in NLP outside of multi-hop QA has been identifying subsets of input tokens to justify decisions.
%For text classification, \citet{lei-etal-2016-rationalizing}, \citet{bastings-etal-2019-interpretable}, and \citet{chen-ji-2020-learning} frame rationales as minimal subsets of input tokens, based on which models can still make the same predictions.
For text classification, \citet{lei-etal-2016-rationalizing}, \citet{bastings-etal-2019-interpretable}, and \citet{chen-ji-2020-learning} frame rationales as minimal subsets of input tokens.
%However, because there are not constraints on the explanations, they may be contradictory to the inputs.
%For text generation, \citet{vafa-etal-2021-rationales} treat subsets of previously generated tokens as a rationale; because enumerating all rationales is intractable, they proposed a greedy algorithm to approximate the maximum likelihood objective.
%\citet{vafa-etal-2021-rationales} similarly treat subsets of previously generated tokens as a rationale in text generation.
%(e.g., in ``the Supreme Court rejected a challenge to the constitutionality of the death penalty,'' the rationale for generating constitutionality is Supreme, Court, and challenge).
For multi-hop QA, where input tokens are too granular a representation for rationales, treating sentences as rationales within long documents leads to the challenges of hierarchical selection and the representation of long documents; both of which we address with \eba.

Outside of using input tokens for rationales, \citet{zhou2020towards} assume rationales take the form of unconstrained text. While flexible, this approach leads to computationally expensive training methods.
Therefore, we constrain rationales to be a set of sentences from given documents, which both accommodates the production of useful intermediate reasoning steps and keeps training tractable. 
%Our method, \eba, finds a different tradeoff between accuracy and efficiency, as necessitated by the use of sentences as rationales.
%For language understanding tasks, \citet{zhou2020towards} assume explanations in the form of free texts, treat them as a latent variable, and train their model with variational expectation maximization.
\vspace*{-5pt}
\paragraph{Unsupervised evidence retrieval.}
A task closely related to our setting (i.e., no access to rationale supervision) is unsupervised evidence retrieval, which searches for sentences relevant to the questions but does not predict answers.
%One way to leverage such retrieval techniques for multi-hop QA is to first apply them for rationale selections and then predict answers based on the extracted rationales.
For example, one could apply \citet{yadav-etal-2019-quick}, \citet{yadav-etal-2020-unsupervised}, \citet{zhao-etal-2021-distantly} and \citet{xu-etal-2021-exploiting-reasoning} to first identify the rationale for a multi-hop QA example and predict an answer based only on the rationale rather than on the entire document, so that the answer prediction is more constrained.
\vspace*{-5pt}
%\paragraph{Set-valued prediction.}
%Correlated k-subset selection (cite stochastic softmax tricks)
%\justin{include or not?}

==> exNLP_acl2023 (Copy)/results.tex <==
\begin{table*}[t]
% \begin{tabular}{lrrrr}
% \toprule
%  & \multicolumn{1}{l}{Sent EM} & \multicolumn{1}{l}{Sent F1} & \multicolumn{1}{l}{Ans EM} & \multicolumn{1}{l}{Ans F1} \\ \midrule
% BERT Blackbox & - & - & - & 67.1 \\
% DecompRC Blackbox & - & - & - & 70.6 \\
% \textsc{Chain} & - & 64.5 & - & 66.0 \\
% \eba \ Base & 35.2 & 67.1 & 53.5 & 66.8 \\
% \eba \ Large & \textbf{42.0} & \textbf{72.5} & \textbf{60.0} & \textbf{74.5} \\ \midrule
% \textsc{Quark} (Sup.) & 60.7 & 87.0 & 67.8 & 81.2 \\
\centering

\begin{tabular}{lccccc}
\toprule
 & & \multicolumn{2}{c}{HotpotQA} & \multicolumn{2}{c}{MuSiQue} \\ 
 &\#Params& \multicolumn{1}{c}{\textbf{Sent F1}} & \multicolumn{1}{c}{Ans F1} & \multicolumn{1}{c}{\textbf{Sent F1}} & \multicolumn{1}{c}{Ans F1} \\ \midrule
% BERT Blackbox & - & - & - & 67.1 \\
% DecompRC Blackbox & - & - & - & 70.6 \\
%TF-IDF & N/A & 27.3 & N/A \\
BM25 & - & 40.5 & - & 12.9 & -\\
\textsc{RAG}-Small &221M& 49.0 & 62.8& 32.0 & 24.2\\
\eba-Small &221M& 67.1 & 66.8 &34.2&25.1\\
\eba & 761M & \textbf{72.5} & 73.5 &\textbf{44.4}&39.1\\ \midrule
\textsc{Chain} (semi-supervised) & 355M & 64.5 & 66.0 & - & -\\ 
SAE (supervised) & 790M  & 87.4 & 80.8 & 75.2 & 52.3\\
\bottomrule
\end{tabular}%
\caption{Performance comparison on predicting rationales and answers on HotpotQA and MuSiQue.}
\label{tab:hotpotqa}
\end{table*}

\begin{table*}[t]
\centering
% \footnotesize
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lrrrrr|rrrrr}
% \toprule
%  & \multicolumn{5}{c|}{FEVER} & \multicolumn{5}{c}{MultiRC} \\ 
%  & \multicolumn{1}{l}{Sent P} & \multicolumn{1}{l}{Sent R} & \multicolumn{1}{l}{Sent F1} & \multicolumn{1}{l}{Ans Acc} & \multicolumn{1}{l|}{Ans F1} & \multicolumn{1}{l}{Sent P} & \multicolumn{1}{l}{Sent R} & \multicolumn{1}{l}{Sent F1} & \multicolumn{1}{l}{Ans Acc} & \multicolumn{1}{l}{Ans F1} \\ \midrule
% BERT Blackbox & - & - & - & 90.2 & 90.2 & - & - & - & 67.7 & 67.3 \\
% \textsc{Faithful} & 84.0 & \textbf{83.5} & 83.8 & 90.6 & 90.6 & 44.4 & 19.9 & 27.5 & 66.7 & 67.7 \\
% \textsc{Diagnostics} & - & - & 56.1 & - & - & - & - & 38.1 & - & - \\
% \eba-Base & 88.2 & 79.3 & 81.5 & 91.8 & 91.6 & 51.7 & 46.4 & 48.4 & 70.1 & 74.3 \\
% \eba-Large & \textbf{90.9} & 81.7 & \textbf{84.1} & \textbf{94.4} & \textbf{94.3} & \textbf{59.4} & \textbf{53.3} & \textbf{55.6} & \textbf{74.2} & \textbf{75.5} \\ \midrule
% \textsc{Faithful}  \ (Sup.) & 91.7 & 91.1 & 91.4 & 91.1 & 91.1 & 74.3 & 33.5 & 46.1 & 69.1 & 67.4 \\
% \textsc{Diagnostics} (Sup.) & 94.4 & 94.2 & 94.4 & 94.4 & 89.7 & 79.9 & 79.0 & 79.4 & 72.2 & 71.7 \\
\begin{tabular}{lrcccc}
\toprule
 & & \multicolumn{2}{c}{FEVER} & \multicolumn{2}{c}{MultiRC} \\ 
 &\#Params& \multicolumn{1}{c}{\textbf{Sent F1}} & \multicolumn{1}{c}{Ans F1} & \multicolumn{1}{l}{\textbf{Sent F1}} & \multicolumn{1}{l}{Ans F1} \\ \midrule
$\mathbb{RU}$-\textsc{Faithful} & 110M & 83.8 & 90.6 & 27.5 & 67.7 \\
$\mathbb{RU}$-\textsc{Diagnostics} & 110M & 56.1 & - & 38.1 & - \\
\textsc{RAG}-Small & 221M & 80.7 &92.0&44.9& 70.0\\
\eba-Small & 221M & 81.5 & 91.6 & 48.4 & 74.3 \\
\eba & 761M & \textbf{84.1} & 94.3 & \textbf{55.6} & 75.5 \\ \midrule
$\mathbb{RS}$-\textsc{Faithful} (supervised) & 110M & 91.4 & 91.1 & 46.1 & 67.4 \\
$\mathbb{RS}$-\textsc{Diagnostics} (supervised) & 110M & 94.4 & 89.7 & 79.4 & 71.7 \\
%WT5 (supervised) & 220M & - & - & - & 77.8 \\
\bottomrule
\end{tabular}%
\caption{Performance comparison on predicting rationales and answers on Eraser-FEVER and Eraser-MultiRC. \eba \ has more parameters due to its use of a seq2seq model for answer generation.}
\label{tab:multirc_fever}
\end{table*}

\section{Results}
\label{sec:results}
% Because the parameter size of \eba-Small is closer than that of \eba\ to the sizes of all compared models, we use \eba-Small when making these performance comparisons.

\paragraph{HotpotQA.} We summarize the results on HotpotQA in Table~\ref{tab:hotpotqa}.
%Compared to the blackbox models whose backbones are BERT-base models, \eba \ Base has a similar accuracy for answer predictions while producing the rationales for how the predictions are made.
%Additionally, by using a much smaller model, \eba \ Base already outperforms \textsc{Chain} by nearly 3 point on identifying rationale while maintaining similar answer accuracy.
%\eba-Small outperforms the best rule-based approach, BM25, by 27 sentence F1 points, suggesting that it has learned to how to select rationales rather than simply performing a lexical match.
\eba-Small outperforms the best unsupervised approach \textsc{RAG}-Small by 18 sentence F1 points, demonstrating superior multi-hop reasoning abilities.
\eba-Small, despite having fewer parameters, outperforms the semi-supervised \textsc{Chain} on predicting rationales and is comparable to \textsc{Chain} on predicting answers.
While \textsc{Chain} explicitly exploits the heuristics used in the data collection process for HotpotQA, \eba-Small \ is able to learn such heuristics in a fully automatic way.
%We also show that \eba \ can benefit from larger pretrained language models.
%By using the largest available RoBERTa model and BART model, we are able to improve sentence F1 score by 5 absolute point and improve answer F1 by 8 absolute point.
Finally, the gap between \eba \ and SAE, a fully supervised method that is given both rationale and answer annotations, remains large.

\paragraph{MuSiQue.} Table~\ref{tab:hotpotqa} shows that \eba-Small is better at both identifying rationales and predicting answers than \textsc{RAG}-Small, the best-performing unsupervised baseline.
Due to the difficulty of MuSiQue, it is harder for an unsupervised method to learn to select rationales -- the gap between the supervised method and the best unsupervised method on this dataset is greater than the gap on HotpotQA.

\paragraph{FEVER}
%Because both Eraser-FEVER and Eraser-MultiRC only involve selecting rationales from a single document, we group the results on the two datasets in Table~\ref{tab:multirc_fever}.
%First of all, even though \eba \ is constrained to only use selected sentences to predict answers, as opposed to BERT Blackbox predicting answers with the entire document, \eba \ still outperforms BERT Blackbox.
We summarize the results on FEVER in Table~\ref{tab:multirc_fever}.
In terms of selecting rationales in an unsupervised manner, \eba-Small outperforms $\mathbb{RU}$-\textsc{Diagnostics}, performs similarly to \textsc{RAG}-Small, and underperforms $\mathbb{RU}$-\textsc{Faithful} by a small margin.
Because FEVER mostly only requires single-hop reasoning, \eba-Small does not improve over the previous methods.
On predicting answers, \eba-Small outperforms $\mathbb{RU}$-\textsc{Faithful} but underperforms \textsc{RAG}-Small.
Compared to the supervised versions of $\mathbb{RS}$-\textsc{Diagnostics} and $\mathbb{RS}$-\textsc{Faithful}, which have access to both the answers and rationales during training, the gap between \eba-Small's and their rationale scores (sentence F1) understandably remains large. 

% Interestingly, \eba-Small is better at predicting answers.
% This may be attributed to the fact that our answer model uses more parameters than the baseline models.
% However, the advantage in number of parameters does not apply to \eba-Small's capacity of selecting rationales --- its encoder is the much smaller distilBERT whereas the encoders of \textsc{Faithful} and \textsc{Diagnostics} are BERT-base.

% When comparing to the state-of-the-art unsupervised methods, both \textsc{Faithful} and \textsc{Diagnostics} are good at one dataset but drastically fail on the other dataset; however, \eba \ is able to consistently perform well on FEVER and MultiRC.
% %Again, by using larger models for parameterization, \eba \ can consistently achieve better results.
% Again, compared to fully supervised methods, \eba \ is worse at identifying rationales but produce comparable answer F1 scores.

\paragraph{MultiRC}
Table~\ref{tab:multirc_fever} shows that \eba-Small outperforms all comparison models including \textsc{RAG}-Small -- the best competing approach without rationale supervision -- by 3.5 sentence F1 points and 4.3 answer F1 points.
%When compared to the supervised methods, \eba-Small is worse at predicting answers and selecting rationales.

% \begin{table}[t]
% \centering
% \footnotesize
% \begin{tabular}{llrrr}
% \toprule
%  &  & \multicolumn{1}{l}{HotpotQA} & \multicolumn{1}{l}{FEVER} & \multicolumn{1}{l}{MultiRC} \\ \midrule
% \multirow{2}{*}{Sent. F1} & \eba & 67.1 & 81.5 & 48.4 \\
%  & \eba+ & \textbf{72.5} & \textbf{84.1} & \textbf{55.6} \\ \midrule
% \multirow{2}{*}{Ans. F1} & \eba & 66.8 & 91.6 & 74.3 \\
%  & \eba+ & \textbf{74.5} & \textbf{94.3} & \textbf{75.5} \\
%  \bottomrule
% \end{tabular}
% \caption{Comparison of \eba \ of different sizes. \eba \ has 205 million parameters, whereas \eba+ has 761 million parameters.}
% \label{tab:scalingup}
% \end{table}

\paragraph{Scaling \eba \ to Larger Models.}
%On all three datasets, by increasing the encoder size from distilBERT to RoBERTa-large and by increasing the sequence-to-sequence model size from BART-base to BART-large, \eba \ can consistently achieve better performance on both selecting rationales and predicting answers.
On all three datasets, by increasing the number of model parameters, \eba \ can consistently achieve better performance. %on both selecting rationales and predicting answers.
Additionally, as the number of reasoning hops increases, \eba \ can more benefit from the larger language models -- compared to \eba-Small, \eba \ has the least improvement on FEVER and had the most improvement on MuSiQue.
%\eba \ can thus benefit from larger, more expressive language models.

==> exNLP_acl2023 (Copy)/setup.tex <==
\section{Experimental Setup}
\label{sec:experiments}
\begin{table}[t]
\centering
\small
\begin{tabular}{p{0.07\linewidth} p{0.04\linewidth} p{0.75\linewidth}}
\toprule
& \cellcolor{blue!15} In          & \cellcolor{blue!15} {\noindent \color{red} \textit{A claim to be verified is that}} \{$x$\} {\noindent \color{red} \textit{We have following facts:}} \{$\bm{z}$\} \\
      & \cellcolor{blue!15} Out                        & \cellcolor{blue!15} {\noindent \color{red} \textit{The claim is thus}} \{supported/refuted\}. \\
BQA  & \cellcolor{green!15} In          & \cellcolor{green!15} {\noindent \color{red} \textit{A claim to be verified is that}} Steve Wozniak designed homes. {\noindent \color{red} \textit{We have following facts:}} Steve Wozniak primarily designed the 1977 Apple II , known as one of the first highly successful mass-produced microcomputers. \\

     & \cellcolor{green!15} Out                        & \cellcolor{green!15} {\noindent \color{red} \textit{The claim is thus}} refuted. \\ \midrule

& \cellcolor{blue!15} In         & \cellcolor{blue!15} {\noindent \color{red} \textit{Question:}} \{$x$\} \texttt{[SEP]} \{$\bm{z}$\} \\
           & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} {\noindent \color{red} \textit{Answer:}} \{$y_1$\} (\{correct/wrong\}) \texttt{[SEP]} {\noindent \color{red} \textit{Answer:}} \{$y_2$\} (\{correct/wrong\}) \texttt{[SEP]} ...  \\
MCQ & \cellcolor{green!15} In         & \cellcolor{green!15} {\noindent \color{red} \textit{Question:}} Name few objects said to be in or on Allan 's desk. \texttt{[SEP]} Opening a side drawer, he took out a piece of paper and his inkpot. \\
           & \cellcolor{green!15} Out                  & \cellcolor{green!15}  {\noindent \color{red} \textit{Answer:}} Eraser  (wrong) \texttt{[SEP]} {\noindent \color{red} \textit{Answer:}} Inkpot (correct) \texttt{[SEP]} {\noindent \color{red} \textit{Answer:}} Pen (correct) \\ \midrule

 & \cellcolor{blue!15} In         & \cellcolor{blue!15} \{$x$\} \texttt{[SEP]} \{$\bm{z}$\} \\
           & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} \{$y$\} \\
EQA & \cellcolor{green!15} In         & \cellcolor{green!15} Which American railroad, located in Southwestern Montana and Idaho, was backed by the Northern Pacific Railway? \texttt{[SEP]} The Gilmore and Pittsburgh Railroad (G\&P), now defunct, was an American railroad located in southwestern Montana and east-central Idaho. \\
           & \cellcolor{green!15} Out                  & \cellcolor{green!15} Gilmore and Pittsburgh Railroad \\
\bottomrule
\end{tabular}%
\caption{Seq-to-Seq Prompt templates for QA examples for FEVER as Boolean QA (BQA), MultiRC as multiple-choice QA (MCQ), and HotpotQA as extractive QA (EQA). Templates are in purple cells, followed by specific examples in green cells. Template keywords are highlighted in {\color{red} \textit{red italics}}.}
\vspace*{-10pt}
\label{tab:conversion}
\end{table}

\paragraph{Datasets and Their Representations.}
We evaluate \eba \ on four multi-hop QA datasets: HotpotQA in the distractor setting~\cite{yang-etal-2018-hotpotqa}, MuSiQue with answerable questions~\cite{trivedi2021musique}, FEVER~\cite{thorne-etal-2018-fever}, and MultiRC~\cite{khashabi-etal-2018-looking}.
HotpotQA and MuSiQue are extractive QA datasets that require reasoning over multiple Wikipedia documents and identifying a span of text as the answer.
In HotpotQA, each example contains ten candidate documents, and we must identify exactly two documents ($|D|=2$) that are relevant.
FEVER is a fact checking dataset that requires verifying claims made based on Wikipedia articles ($|D|=1$).
MultiRC is a multiple-choice QA dataset collected from diverse sources of documents including narrative stories and news articles, and their questions can only be answered by reasoning over multiple sentences ($|D|=1$).
%and thus do not need document selection.
Unlike conventional multi-choice tasks~\cite{lai-etal-2017-race,richardson-etal-2013-mctest}, MultiRC does not pre-specify the number of correct answer choices, resulting in a more challenging setting.
For FEVER and MultiRC, we consider the ERASER version~\cite{deyoung-etal-2020-eraser}, where rationale annotations are made cleaner and evaluation metrics are provided.
% Of the three datasets, only HotpotQA has more than one documents, and thus no document selection is performed for the other two datasets.

In Table~\ref{tab:conversion}, we demonstrate how to convert QA examples of these three datasets to a natural language prompt format~\cite{brown2020language}.
In FEVER, a claim $x$ needs to be classified as whether it is supported (1) or refuted (0) given the accompanying documents $D$.
% Inspired by prompting~, instead of directly inputting $x, \bm{z}$ and outputting $0/1$, we connect them with instructional prompts.
For MultiRC, there is a varying number of choices per example, and an unknown number of the choices is correct; we stack all answer choices attached with their truth values as outputs to supervise the model.
% We further note that determining the truth value of one answer choice may not require all sentences in the rationale; therefore, knowing the truth value of one answer choice does not have enough information to inform the entire rationale.
% For this reason, we stack all answer choices attached with their truth values as outputs to supervise the model.
Finally, extractive QA can naturally be formulated as a text-to-text problem, where the input is $x$ \texttt{[SEP]} $\bm{z}$, and the output is $y$.

\paragraph{Metrics and Comparison Systems.}
% We follow the metrics proposed in \citet{yang-etal-2018-hotpotqa,glockner-etal-2020-think}.
% When evaluating answers, we compute exact match (EM) and F1 scores.
% For HotpotQA, F1 scores are averaged over samples.
% For FEVER and MultiRC, macro-averaged F1 scores are used.
% When evaluating rationales, we compute precision (P), recall (R), exact match, and sample-based F1 scores. 
% Finally, to determine the best overall system, we calculate joint EM and joint F1 for answers and rationales.
We compute F1 scores for rationale and document selection, and answer prediction.
F1 scores for rationales are computed at the sentence level.
Because the three QA datasets are in different formats, F1 scores for answers are computed differently.
For extractive QA, F1 scores are computed at the token level for the answer spans.
For Boolean QA and multiple-choice QA, F1 scores measure categorical answers.

For each dataset, we compare to (1) state-of-the-art approaches that require no rationale supervision and (2) at least one fully supervised method (i.e., answers and rationales available for training). The latter provides an upper bound on performance.\\
%Additionally, we compare to blackbox systems, which helps us to measure if we need to sacrifice accuracy performance for explainability.
\noindent
%\textbf{-- On HotpotQA}, to the best of our knowledge, no existing learning-based systems\footnote{We cannot apply \textsc{Diagnostics} and \textsc{Faithful} to HotpotQA because they only work for categorical $y$ (i.e., Yes/No answers, multiple-choice answers, etc).} are unsupervised.
\textbf{-- On HotpotQA and MuSiQue}, we compare to a rule-based approaches, BM25, and $\textsc{RAG}$~\cite{NEURIPS2020_6b493230} as unsupervised baselines.
We note that $\textsc{RAG}$ only performs document-level retrieval, and therefore its current form cannot be directly applied to identifying sentence-level rationales.
We modify $\textsc{RAG}$ to treat a sentence as a document, and at inference we take the top-3 sentences to be the rationale as it results in the highest sentence F1 scores.
For fair comparison, we parameterize $\textsc{RAG}$ in the same way as we parameterize \eba.
We also consider a semi-supervised approach -- \textsc{Chain}~\cite{chen2019multi}; they assume no access to gold rationale annotations and supervise their model on silver rationales produced with external entity taggers.
The fully supervised system we consider is SAE~\cite{tu2020select}.
Both \textsc{Chain} and SAE use RoBERTa-large as sentence encoders.\\
%We compare to a BART model and DecompRC~\cite{min-etal-2019-multi} as the blackbox systems.
%To eliminate the effect that text-to-text models may perform worse at span prediction tasks, we also make a reference to the BERT-base model in \citet{min-etal-2019-multi}.
\noindent
\textbf{-- On FEVER and MultiRC}, we also compare to $\textsc{RAG}$ as an unsupervised baseline (predicting top-2 sentences for MultiRC, and top-1 sentence for FEVER).
Additionally, we consider diagnostics-guided explanation generation (\textsc{Diagnostics}) \cite{atanasova2022diagnostics} and faithful rationales (\textsc{Faithful}) \cite{glockner-etal-2020-think}.
Both of these methods have two variants -- one trained with rationale supervision (denoted by $\mathbb{RS}$-*) and the other trained without rationale annotations (denoted by $\mathbb{RU}$-*).
On MultiRC, We also compare to WT5~\cite{DBLP:journals/corr/abs-2004-14546}.
%Since FEVER and MultiRC have rather short contexts, we take BERT from~\citet{glockner-etal-2020-think} as the blackbox system.

\paragraph{Implementation and Hyperparameters.}
%We test \eba \ with both base and large language models.
%First, for the base version, we take distilBERT~\cite{Sanh2019DistilBERTAD} to be the encoder, which is only half of the size as the base model of BERT.
%We load the pretrained weights from a sentenceBERT model\footnote{https://huggingface.co/sentence-transformers/all-distilroberta-v1}\cite{reimers-gurevych-2019-sentence}.
%The seq2seq model we use to parameterize $p(y|\bm{z}, x)$ is BART-base~\cite{lewis-etal-2020-bart}.
%For the large version, we use RoBERTa-large for computing $\text{emb}(\cdot)$ and BART-large for the answer model.
We test \eba \ with language models of both small and large sizes.
For the small version (\eba-Small), we use distilBERT~\cite{Sanh2019DistilBERTAD} as the encoder and BART-base as the seq2seq model.
For the large version (\eba), we use RoBERTa-large as the encoder and BART-large as the seq2seq model.
We only test \textsc{RAG} in the small version.

We implement \eba \ with Hugging Face Transformers~\cite{wolf-etal-2020-transformers}.
We perform grid search with learning rates \{5e-6, 1e-5, 2e-5\} and batch sizes \{2,4,8,16\} for both \eba \ and \textsc{RAG}.
We train our system for 3 epochs for HotpotQA and 5 epochs for the other three datasets.
We warm up the learning rate with first 10\% examples.
We choose the checkpoint that has the highest answer F1 score on the validation set.
We consider rationales up to four sentences for HotpotQA and rationales up to three sentences for the other datasets.
%
%Finally, we let $|\mathcal{S}_d|=10$ and $|\mathcal{S}_{\bm{z},d}|=9$ for HotpotQA and $|\mathcal{S}_{\bm{z}}|=80$ for MultiRC.
Finally, we take $S^{10}$ and $S_{\bm{d}}^9$ for HotpotQA and $S_{\bm{d}}^{80}$ for MultiRC.
Because we remove rationales whose sentences are not contiguous in FEVER, we are able to compute the exact likelihood without top-k sampling.

==> old_method.tex <==
\section{Method}
% \label{fig:generative}
% \end{figure}
% \begin{figure}[t]
%   \begin{center}
%   \scalebox{.85}{
%     \begin{tikzpicture}
%     \node[latent] (d) {$D_i$};
%     \factor[left=of d, xshift=-0.2cm] {dp} {} {} {} ;
%     \node[latent, right=of d] (z) {$Z_i^j$};
%     \factor[left=of z, xshift=-0.1cm] {zp} {} {} {} ;
%     \node[obs, right=of z] (y) {$Y$};
%     \factor[left=of y, xshift=-0.1cm] {yp} {} {} {} ;
%     \edge {dp} {d};
%     \edge {d} {z};
%     \edge {z} {y};
%     \plate [inner sep=.23cm,xshift=-.1cm,yshift=.2cm] {plate2} {(z)} {$J$};
%     \plate [inner sep=0.25cm,xshift=-.15cm,yshift=.2cm] {plate1} {(plate2)(d)} {$I$};
%     \end{tikzpicture}
%     }
%   \end{center}
% \caption{The graphical model for the generative process for multi-hop QA when $m=2$. Because every other random variable depends on $X$, we omit it for the sake of simplicity.}
% \label{fig:generative}
% \end{figure}

% \begin{figure}[!t]
%     \textbf{\textit{{\small Parallel Reasoning:}}}\\
%     \framebox{
%     \parbox{0.45\textwidth}{
%     \small
%     \textbf{Q:} Are Hattiesburg–Laurel Regional Airport and Wilmington International Airport both located in North Carolina? \noindent \smallskip \newline
%     \textbf{Document A, Wilmington International Airport:} \newline
%     Wilmington International Airport is a public airport located just north of Wilmington, North Carolina. [$\dotsc$]\newline
%     \textbf{Document B, Hattiesburg–Laurel Regional Airport:} \newline
%     Hattiesburg–Laurel Regional Airport, also Airport City, is a public airport in Jones County, Mississippi. [$\dotsc$]\smallskip \newline
%     \textbf{A:} No}
%     }\vspace*{2pt}
%     \textbf{\textit{{\small Sequential Reasoning:}}}\\
%     \framebox{
%     \parbox{0.45\textwidth}{
%     \small
%     \textbf{Q:} Which team does the player named 2015 Diamond Head Classic’s MVP play for? \noindent \smallskip \newline
%     \textbf{Document A, 2015 Diamond Head Classic:} \newline
%     [$\dotsc$] Buddy Hield was named the tournament’s MVP.\newline
%     \textbf{Document B, Buddy Hield:} \newline
%     Buddy Hield is a Bahamian professional basketball player for the Sacramento Kings of the NBA. [$\dotsc$]\smallskip \newline
%     \textbf{A:} Sacramento Kings}
%     }
%     \caption{Demonstrations on when parallel and sequential reasoning are applied in multi-hop reasoning. Irrelevant sentences are removed from the documents.} \label{fig:example}
% \end{figure}
% \begin{figure}[t]
%   \begin{center}
%   \scalebox{.85}{
%     \begin{tikzpicture}
%     \node[obs] (x) {$X$};
%     \node[latent, right=of x] (z) {$Z$};
%     \node[obs, right=of z] (y) {$Y$};
%     \edge {x} {z};
%     \edge {z} {y};
%     \draw[->] (x) to[bend left] (y);
%     \end{tikzpicture}
%     }
%   \end{center}
% \caption{The graphical model for the generative process for multi-hop QA when $|\bm{D}|=1$.}
% \label{fig:generative}
% \end{figure}
% We now describe \eba, an explainable approach for multi-hop QA that requires no rationale supervision.


\begin{figure}
    \centering
    \small
    \framebox{
    \parbox{0.45\textwidth}{
    \small
    \textbf{Q:} A medieval fortress in Dirleton, East Lothian, Scotland borders on the south side of what coastal area? \noindent \smallskip \newline
    \textbf{Document A, Yellowcraig:} \newline
    \support{Yellowcraig, less commonly known as Broad Sands Bay, is a coastal area of forest, beach and grassland in East Lothian, south-east Scotland.} Yellowcraig is partly within the Firth of Forth Site of Special Scientific Interest (SSSI). \support{It is bordered to the north by the Firth of Forth, to the south by the village of Dirleton and Dirleton Castle, to the east by the North Berwick West Links golf course, and to the west by the Archerfield Estate and Links golf courses.}\newline
    \textbf{Document B, Dirleton Castle:} \newline
    \support{Dirleton Castle is a medieval fortress in the village of Dirleton, East Lothian, Scotland.} It lies around 2 mi west of North Berwick, and around 19 mi east of Edinburgh. The oldest parts of the castle date to the 13th century, and it was abandoned by the end of the 17th century.\smallskip \newline
    \textbf{A:} Yellowcraig}
    }
    \caption{A multi-hop QA example. The sentences used to derive the answer are highlighted in \support{blue italics}.}
    \label{fig:multihop_example}
\end{figure}
Figure~\ref{fig:multihop_example} shows a multi-hop QA example, which starts with a question, accompanied by one or multiple supporting documents, and an answer can be derived from a set of sentences in the documents.

We start with multi-hop reasoning over a single document.
Then, we show by adding a document selection module, \eba \ can easily be extended to reason over multiple documents.
Formally, a multi-hop QA example consists of a question $X$, a document $D$, and an answer $Y$.
An explainable method for multi-hop QA not only predicts $Y$, but also generates a rationale $Z \in \mathcal{P}(D)$, which is a minimal set of sentences in $D$ from which $Y$ can be derived.
Hops are defined at the sentence level; if a question requires reasoning over multiple sentences to reach the answer, then we consider it to be a multi-hop QA problem.

The goal of multi-hop QA is to produce a probability distribution over answers $Y$ to questions $X$, defined by $P(Y|X)$.
In order to produce answers $Y$, \eba \ first identifies unobserved rationales $Z$ given question $X$, then chooses answers $Y$ given both $X$ and $Z$.
This yields the joint distribution
\begin{align*}
    P(Y,Z|X) = P(Z|X)P(Y|X,Z).
\end{align*}
%illustrated in Figure \ref{fig:generative}

% The goal of multi-hop QA is to produce a probability distribution over answers $Y$, defined by $P(Y|X)$.
% \eba \ assumes a data generating process shown in Figure~\ref{fig:generative}, where rationales $Z$ are unobserved but directly affect $Y$.
% According this generative process, \eba \ proceeds in two stages:
% \begin{align*}
%     P(Y,Z|X) = P(Z|X)P(Y|X,Z)
% \end{align*}
This factorization naturally provides explainability -- in the first phase, \eba \ identifies rationales $Z$ based on the information contained in $X$; in the second phase, \eba \ derives answers $Y$ from both questions $X$ and rationales $Z$.
Our goal is to train \eba \ to produce high $P(Y|X,Z)$ for correct rationales and low $P(Y|X,Z)$ for incorrect rationales.
% Formally, a multi-hop QA example consists of a question $X$, a set of documents $\bm{D}$, and an answer $Y$.
% We assume that each task pre-specifies the number of relevant documents to be $m$.
% An explainable method not only predicts $Y$, but also generates a rationale $Z \in \mathcal{P}(\bm{D})$, which is a minimal set of sentences in the $m$ documents from which $Y$ can be derived.
% We first describe \eba \ for $|\bm{D}|=1$, where there is no need for document selection.
% We then show and generalize it to reasoning over multiple documents.

% Here, we consider exactly two documents are relevant to the question, but \eba \ can be easily extended to more documents.
% We assume there are unobserved variables $D_1$ and $D_2$, representing two supporting documents.
% Further, there are another two unobserved variables $Z_1$ and $Z_2$, representing sets of sentences selected from $D_1$ and $D_2$, respectively.
% We specify the generative process for multi-hop QA in Figure~\ref{fig:generative}, where only question $X$ and answer $Y$ are observed.
% Because all the remaining variables condition on $X$, we omit it from the graphical model.

% Without document selection, the generative model proceeds in two phases.
% At the first phase, the model selects documents, which naturally leads to a model design choice -- whether to make an independence assumption between the two documents.
% With the independence assumption, each document can be considered individually; therefore, selecting documents has a low complexity that is linear to the number of documents.
% To illustrate how our design choice is made, we first differentiate two types of multi-hop reasoning in Figure~\ref{fig:example}.
% To answer the first question, it is possible to independently identify what documents may be needed to derive an answer.
% Thus, selecting each of the two documents can be done in parallel.
% However, in the second question, it is not possible to identify Document B without knowing the information in Document A.
% Thus, answering the second question requires reasoning about the two documents in a specific order.
% To capture this sequential nature of multi-hop reasoning, we condition $D_2$ on both $X$ and $D_1$, so that \eba \ has enough expressive power to answer the questions that requires performing sequential reasoning.

% At the second stage, the model chooses a set of sentences from the documents.
% Because we already take into account the relation between multiple documents at the first stage, $Z_2$ is made independent of $Z_1$.
% We further point out that the number of choices of $Z_1$ and $Z_2$ are exponential to the number of sentences in $D_1$ and $D_2$, respectively.
% For this reason, approximating distributions over $Z_1$ and $Z_2$ separately has a lower complexity than approximating a distribution over $Z_1 \times Z_2$.
% Finally, answer $Y$ is predicted with both $Z_1$ and $Z_2$.
% In summary, our probabilistic model places a distribution over $(D_1, D_2, Z_1, Z_2, Y)$ and factorizes according to the three phases as follows:
% \begin{align*}
%     P(D_1, D_2, Z_1, Z_2, Y) = &P(D_1)P(D_2|D_1) \\
%     \cdot &P(Z_1|D_1)P(Z_2|D_2) \\
%     \cdot &P(Y|Z_1, Z_2)
% \end{align*}

\subsection{Parameterization}
We now turn to how \eba \ parameterizes each model.
We first describe the parameterization for the rationale model $P(Z|X)$.
Let $\text{emb}: \mathcal{V}^* \rightarrow \mathbb{R}^n$ be an embedding function that maps a sequence of text $\mathcal{V}^*$ to a real-valued vector of $n$ dimensions, where $\mathcal{V}$ is a vocabulary.
%Let $W: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a linear layer,
Let $\bm{w}$ be an $n$-dimensional vector,
\begin{equation*}
    %P(Z=z|X) = \frac{e^{W(\text{emb}(z))}}{\sum_{z'} e^{W(\text{emb}(z'))}}.
    P(Z=z|X=x) \propto \text{exp}(\langle \bm{w}, \text{emb}(z, x)\rangle)
\end{equation*}
Because there are exponentially many possible rationales, computing an embedding for every one of them is intractable.
Instead, we compute an embedding for each sentence $s \in D$.
To obtain the rationale embedding of a particular $z$, we aggregate sentence embeddings $\text{emb}(s)$ for every sentence $s \in z$ via mean.
In practice, $\text{emb}(\cdot)$ is implemented with bidirectional encoders such as BERT~\cite{devlin-etal-2019-bert}.
The input we feed to the encoders is $D$, with an [UNK] token inserted before each sentence: ``$X$ [SEP] [UNK] $s_1$ [UNK] $s_2$ ... [UNK] $s_{|D|}$''.
We take the last hidden state of each [UNK] token to be the embedding for the sentence following right after that [UNK] token.
Therefore, computing $P(Z|X)$ only requires one forward pass of the encoders.
To summarize, compared to \citet{atanasova2022diagnostics} where all sentences in a rationale are all predicted in a fully independent way, we are able to add dependency between sentences with little overhead via a parameterization trick.

\begin{table}[t]
\centering
\small
\begin{tabular}{p{0.07\linewidth} p{0.04\linewidth} p{0.75\linewidth}}
\toprule
& \cellcolor{blue!15} In          & \cellcolor{blue!15} {\noindent \color{red} \textit{A claim to be verified is that}} $X$ {\noindent \color{red} \textit{We have following facts:}} $Z$ \\
      & \cellcolor{blue!15} Out                        & \cellcolor{blue!15} {\noindent \color{red} \textit{The claim is thus}} \{supported/refuted\}. \\
BQA  & \cellcolor{green!15} In          & \cellcolor{green!15} {\noindent \color{red} \textit{A claim to be verified is that}} Steve Wozniak designed homes. {\noindent \color{red} \textit{We have following facts:}} Steve Wozniak primarily designed the 1977 Apple II , known as one of the first highly successful mass-produced microcomputers. \\

     & \cellcolor{green!15} Out                        & \cellcolor{green!15} {\noindent \color{red} \textit{The claim is thus}} refuted. \\ \midrule

& \cellcolor{blue!15} In         & \cellcolor{blue!15} {\noindent \color{red} \textit{Question:}} $X$ [SEP] $Z$ \\
           & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} {\noindent \color{red} \textit{Answer:}} $Y_1$ (\{correct/wrong\}) [SEP] {\noindent \color{red} \textit{Answer:}} $Y_2$ (\{correct/wrong\}) [SEP] ...  \\
MCQ & \cellcolor{green!15} In         & \cellcolor{green!15} {\noindent \color{red} \textit{Question:}} Name few objects said to be in or on Allan 's desk. [SEP] Opening a side drawer, he took out a piece of paper and his inkpot. \\
           & \cellcolor{green!15} Out                  & \cellcolor{green!15}  {\noindent \color{red} \textit{Answer:}} Eraser  (wrong) [SEP] {\noindent \color{red} \textit{Answer:}} Inkpot (correct) [SEP] {\noindent \color{red} \textit{Answer:}} Pen (correct) \\ \midrule

 & \cellcolor{blue!15} In         & \cellcolor{blue!15} $X$ [SEP] $Z$ \\
           & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} $Y$ \\
EQA & \cellcolor{green!15} In         & \cellcolor{green!15} Which American railroad, located in Southwestern Montana and Idaho, was backed by the Northern Pacific Railway? [SEP] The Gilmore and Pittsburgh Railroad (G\&P), now defunct, was an American railroad located in southwestern Montana and east-central Idaho. \\
           & \cellcolor{green!15} Out                  & \cellcolor{green!15} Gilmore and Pittsburgh Railroad \\
\bottomrule
\end{tabular}%
\caption{Example conversions from QA examples to text-to-text examples for Boolean QA (BQA), multiple-choice QA (MCQ), and extractive QA (EQA). Templates are in purple cells, followed by specific examples in green cells. Template keywords are highlighted in {\color{red} \textit{red italics}}.}
\label{tab:conversion}
\end{table}

We then describe the parameterization for the answer model $P(Y|X, Z)$.
Because \citet{khashabi-etal-2020-unifiedqa} show that text-to-text models can handle QA tasks of all formats, they become a natural choice for parameterizing $P(Y|Z_1, Z_2)$.
Examples of such models are BART~\cite{lewis-etal-2020-bart} and T5~\cite{2020t5}.
The exact parameterization of the answer model is task-dependent.
In Table~\ref{tab:conversion}, we demonstrate how to convert QA examples of different forms to text-to-text examples.
For Boolean QA, we take the problem of fact checking as an example, in which a claim $X$ needs to be classified as whether it is supported (0) or refuted (1) with the accompanying documents $\bm{D}$.
Inspired by prompting~\cite{brown2020language}, instead of directly inputting $X, Z$ and outputting $0/1$, we connect them with instructional prompts.
For multiple-choice QA, we consider a general case where there is a varying number of choices per example, and an unknown number of the choices is correct.
We note that determining the truth value of one answer choice may not require all sentences in the rationale; therefore, knowing the truth value of one answer choice does not have enough information to inform the entire rationale.
For this reason, we stack all answer choices attached with their truth values as outputs to supervise the model.
Finally, extractive QA can naturally be formulated as a text-to-text problem, where the input is $X$ [SEP] $Z$, and the output is $Y$.

\subsection{Training \& Inference}
To learn an explainable multi-hop QA system, \eba \ maximizes the likelihood function $\mathcal{L}(\cdot)$ with respect to parameters $\theta$ for all training examples:
\begin{equation*}
    \mathcal{L(\theta)} = \text{log} \sum_{Z} P_\theta(Z|X) P_\theta(Y|X, Z).
\end{equation*}
We note that even though $P_\theta(Z|X)$ can be computed efficiently with our parameterization trick, $P_\theta(Y|X, Z)$ requires encoder-decoder models to perform $|Z|$ forward passes.
Thus, the exact computation of $\mathcal{L(\theta)}$ will still be intractable when the number of sentences in $D$ is large.
We thus approximate this objective by
\begin{equation*}
    \mathcal{L(\theta)} \approx \text{log} \sum_{z\in \mathcal{S}} P_\theta(Z|X) P_\theta(Y|X, Z),
\end{equation*}
where $\mathcal{S} = \argtopk_{Z} P_\theta(Z|X)$.
At test time, \eba \ chooses the rationale by
\begin{equation*}
    z=\argmaxB_{Z} P_\theta(Z|X).
\end{equation*}
Therefore, rationales are selected by conditioning only on the questions without peeking at the answers.
Finally, when predicting the answer, we generate an answer by performing greedy search on $P(Y|Z=z, X)$ for span-based QA.
For Boolean QA or multiple-choice QA, we normalize over different answer choices and take the answer to be $\argmaxB_{Y}P(Y|Z=z, X)$.

\begin{figure}[t]
  \begin{center}
  \scalebox{.85}{
    \begin{tikzpicture}
    \node[obs] (x) {$X$};
    \node[latent, right=of x] (d) {$D_1$};
    \node[latent, below=of d] (dd) {$D_2$};
    \node[latent, right=of d] (z) {$Z_1$};
    \node[latent, right=of dd] (zz) {$Z_2$};
    \node[obs, right=of z] (y) {$Y$};
    \edge {x} {d};
    \edge {x} {dd};
    \draw[->] (x) to[bend left] (z);
    \draw[->] (x) to[bend left] (y);
    \edge {x} {zz};
    \edge {d} {dd};
    \edge {d} {z};
    \edge {dd} {zz};
    \edge {z} {y};
    \edge {zz} {y};
    \end{tikzpicture}
    }
  \end{center}
\caption{The graphical model is updated to handle multi-hop QA for $m=2$.}
\label{fig:generative2}
\end{figure}
\subsection{Reasoning over Multiple Documents}
Resolving queries may often involve reasoning over large contexts involving multiple documents. We extend \eba \ to handle multiple documents by making two modifications to the previous setup: single documents $D$ become a set of documents $\bm{D}$, and not every document in $\bm{D}$ is relevant to the question.
We assume the number of relevant documents $m$ is pre-specified by each task.
Here, we describe how to extend \eba \ to $m=2$.
We let $D_1$ and $D_2$ to be the first and the second relevant documents, respectively.
In a rationale $Z=(Z_1, Z_2)$, $Z_1 \subseteq D_1$ and $Z_1 \subseteq D_1$.
We update the graphical model in Figure~\ref{fig:generative2}.
With the new data generating process, \eba \ proceeds in three stages (with $X$ omitted for the sake of brevity),
\begin{align*}
    P(D_1, D_2, Z_1, Z_2, Y) = &P(D_1)P(D_2|D_1) \\
    \cdot &P(Z_1|D_1)P(Z_2|D_2) \\
    \cdot &P(Y|Z_1, Z_2).
\end{align*}
The only addition is \eba \ now starts with document selection.
After two documents are chosen, we repeat the procedure described in the previous section.
We note that, because we want to optimally trade off between accuracy and efficiency, we only consider the dependency between documents in the first stage and assume documents are independent from each other in the second stage.
We show that, with a few tweaks \eba \ can be extended to reason over multiple documents.

\paragraph{Parameterization for the Document Model $P(D_1, D_2|X)$.}
Let $f: D_1 \times D_2 \rightarrow \mathbb{R}$. We assume
\begin{equation*}
    P(D_1, D_2) \propto \exp(f(D_1, D_2)).
\end{equation*}
Because computing an embedding for every pair of documents take quadratic time, we combine two documents in the embedding space via Siamese networks~\cite{reimers-gurevych-2019-sentence}.
Let $\text{e}_{D_1}=\text{emb}(D_1)$ and $\text{e}_{D_2}=\text{emb}(D_2)$, and $[\cdot]$ be a concat operator:
\begin{equation*}
\text{emb}([D_1, D_2]) \approx [\text{e}_{D_1},\text{e}_{D_2},|\text{e}_{D_1}-\text{e}_{D_2}|].
\end{equation*}
Let $\text{MLP}: \mathbb{R}^{3n} \rightarrow \mathbb{R}$ be a multilayer perceptron,
\begin{equation*}
    f(D_1, D_2) = \text{MLP}(\text{emb}([D_1, D_2])).
\end{equation*}
Finally, $P(D_1, D_2|X)$ is normalized over document pairs.
Document embeddings can be obtained almost for free by reusing the computation in the rationale model, where we input the encoders with a document to get an embedding for every sentence.
We append a [CLS] token to the left of the original input and use the last hidden state of this token to be the document embedding.
We note that the encoders can only accept inputs shorter than a fixed length (e.g., 512 tokens).
To address this limitation, we partition documents into slices of $m$ sentences and compute the embbeding for each slice individually.
We denote a slice for a document $D$ as $D^{i:j}$ that starts at the $i$th sentence and ends before the $j$th sentence.
Let $i \in \text{range}(0, |D|, p)$, we approximate $\text{emb}(D)$ by the following aggregation,
\begin{equation*}
    \text{emb}(D) \approx \lfloor \frac{|D|}{m}\rfloor \sum_i \text{emb}(D^{i:i+p}).
\end{equation*}
\paragraph{Training \& Inference}
We describe approximation of the updated likelihood function.
Let $\mathcal{S}_d = \argtopk_{D_1,D_2} P_\theta(D_1, D_2)$.
Let $z_d=(z_1, z_2)$ be a rationale from a given pair of documents $d=(d_1, d_2)$, and $\mathcal{S}_{z, d} = \argtopk_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2)$.
Then,
\begin{equation*}
    \mathcal{L(\theta)} \approx \text{log} \sum_{d\in \mathcal{S}_d} \sum_{z_d\in \mathcal{S}_{z, d}} P_\theta(Y, Z_1, Z_2, D_1, D_2).
\end{equation*}
%\justin{important to emphasize not using posterior}
At test time, we choose a pair of documents by
\begin{equation*}
    d_1, d_2 = \argmaxB_{D_1, D_2} P_\theta(D_1, D_2).
\end{equation*}
Then, we choose a rationale by
\begin{equation*}
    z=\argmaxB_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2).
\end{equation*}
Finally, predicting answers remains unchanged.
% We first consider parametering the document models.
% %Because $P(D_1)P(D_2|D_1)=P(D_2)P(D_1|D_2)$, to avoid symmetric document pairs, instead of identifying the two documents in a sequential manner, we assume
% Let $f: D_1 \times D_2 \rightarrow \mathbb{R}$. We assume
% \begin{equation*}
%     P(D_1, D_2) \propto e^{f(D_1, D_2)}.
% \end{equation*}
% Let $\text{emb}: \bm{T} \rightarrow \mathbb{R}^n$ be an embedding function that maps a text sequence $\bm{T}$ to a real-valued vector of $n$ dimensions.
% Because computing the exact embedding for every pair of documents is computationally expensive, we combine two documents in the embedding space via Siamese networks~\cite{reimers-gurevych-2019-sentence}.
% Let $\text{e}_{D_1}=\text{emb}(D_1)$ and $\text{e}_{D_2}=\text{emb}(D_2)$, and $[\cdot]$ be a concat operator:
% \begin{equation*}
% \text{emb}([D_1, D_2]) \approx [\text{e}_{D_1},\text{e}_{D_2},|\text{e}_{D_1}-\text{e}_{D_2}|].
% \end{equation*}
% Let $\text{MLP}: \mathbb{R}^{3n} \rightarrow \mathbb{R}$ be a multilayer perceptron,
% \begin{equation*}
%     f(D_1, D_2) = \text{MLP}(\text{emb}([D_1, D_2])).
% \end{equation*}
% Finally, $P(D_1, D_2)$ is normalized over document pairs.
% In practice, $\text{emb}(\cdot)$ is implemented with bidirectional encoders such as BERT~\cite{devlin-etal-2019-bert}.
% To obtain an embedding for a document, we feed ``[CLS] $X$ [SEP] $D$'' into the encoders and take the final state of the [CLS] token as the embedding.
% We note that the encoders can only accept inputs shorter than a fixed length (e.g., 512 tokens).
% To address this limitation, we partition documents into slices of $m$ sentences and compute the embbeding for each slice individually.
% We denote a slice for a document $D$ as $D^{i:j}$ that starts at the $i$th sentence and ends before the $j$th sentence.
% Let $i \in \text{range}(0, |D|, p)$, we approximate $\text{emb}(D)$ by the following aggregation,
% \begin{equation*}
%     \text{emb}(D) \approx \lfloor \frac{|D|}{m}\rfloor \sum_i \text{emb}(D^{i:i+p}).
% \end{equation*}

% We then turn to parameterization of the rationale models.
% Since we let $P(Z_1|D_1)$ and $P(Z_2|D_2)$ share the same parameterization, we describe a general model $P(Z|D)$.
% $Z$ consists of all sentence combinations in $D$.
% %Let $\text{emb}_Z: Z \rightarrow \mathbb{R}^n$ and $W: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a linear layer,
% Let $W: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a linear layer,
% \begin{equation*}
%     P(Z=z|D) = \frac{e^{W(\text{emb}(z))}}{\sum_{z'} e^{W(\text{emb}(z'))}}.
% \end{equation*}
% %$\text{emb}_Z(\cdot)$ is also implemented with bidirectional encoders.
% For efficiency, we reuse the computation from the document models.
% Specifically, instead of feeding ``[CLS] $X$ [SEP] $D$'' to an encoder, we modify it to be ``[CLS] $X$ [SEP] [UNK] $D^1$ [UNK] $D^2$ ... [UNK] $D^{|D|}$''.
% That is, we insert a [UNK] token before each sentence and take the last hidden state of the token as the sentence embedding.
% Again, computing the exact embedding for every rationale $z$ is intractable.
% Options for approximating the embedding for $z$ are to combine individual sentence embeddings by max-pooling, sum, and mean.
% We choose to use mean, but they all lead to similar performance.

% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{p{0.07\linewidth} p{0.04\linewidth} p{0.75\linewidth}}
% \toprule
% & \cellcolor{blue!15} In          & \cellcolor{blue!15} {\noindent \color{red} \textit{A claim to be verified is that}} $X$ {\noindent \color{red} \textit{We have following facts:}} $Z$ \\
%       & \cellcolor{blue!15} Out                        & \cellcolor{blue!15} {\noindent \color{red} \textit{The claim is thus}} \{supported/refuted\}. \\
% BQA  & \cellcolor{green!15} In          & \cellcolor{green!15} {\noindent \color{red} \textit{A claim to be verified is that}} Steve Wozniak designed homes. {\noindent \color{red} \textit{We have following facts:}} Steve Wozniak primarily designed the 1977 Apple II , known as one of the first highly successful mass-produced microcomputers. \\

%      & \cellcolor{green!15} Out                        & \cellcolor{green!15} {\noindent \color{red} \textit{The claim is thus}} refuted. \\ \midrule

% & \cellcolor{blue!15} In         & \cellcolor{blue!15} {\noindent \color{red} \textit{Question:}} $X$ [SEP] $Z$ \\
%            & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} {\noindent \color{red} \textit{Answer:}} $Y_1$ (\{correct/wrong\}) [SEP] {\noindent \color{red} \textit{Answer:}} $Y_2$ (\{correct/wrong\}) [SEP] ...  \\
% MCQ & \cellcolor{green!15} In         & \cellcolor{green!15} {\noindent \color{red} \textit{Question:}} Name few objects said to be in or on Allan 's desk. [SEP] Opening a side drawer, he took out a piece of paper and his inkpot. \\
%            & \cellcolor{green!15} Out                  & \cellcolor{green!15}  {\noindent \color{red} \textit{Answer:}} Eraser  (wrong) [SEP] {\noindent \color{red} \textit{Answer:}} Inkpot (correct) [SEP] {\noindent \color{red} \textit{Answer:}} Pen (correct) \\ \midrule

%  & \cellcolor{blue!15} In         & \cellcolor{blue!15} $X$ [SEP] $Z$ \\
%            & \cellcolor{blue!15} Out                  & \cellcolor{blue!15} $Y$ \\
% EQA & \cellcolor{green!15} In         & \cellcolor{green!15} Which American railroad, located in Southwestern Montana and Idaho, was backed by the Northern Pacific Railway? [SEP] The Gilmore and Pittsburgh Railroad (G\&P), now defunct, was an American railroad located in southwestern Montana and east-central Idaho. \\
%            & \cellcolor{green!15} Out                  & \cellcolor{green!15} Gilmore and Pittsburgh Railroad \\
% \bottomrule
% \end{tabular}%
% \caption{Example conversions from QA examples to text-to-text examples for Boolean QA (BQA), multiple-choice QA (MCQ), and extractive QA (EQA). Templates are in purple cells, followed by specific examples in green cells. Template keywords are highlighted in {\color{red} \textit{red italics}}.}
% \label{tab:conversion}
% \end{table}

% Last but not least, because \citet{khashabi-etal-2020-unifiedqa} show that text-to-text models can handle QA tasks of all formats, they become a natural choice for parameterizing $P(Y|Z_1, Z_2)$.
% Examples of such models are BART~\cite{lewis-etal-2020-bart} and T5~\cite{2020t5}.
% The exact parameterization of the answer model is task-dependent.
% In Table~\ref{tab:conversion}, we demonstrate how to convert QA examples of different forms to text-to-text examples.
% %It is worth noting that we have gold labels to supervise the answer model.
% For Boolean QA, we take the problem of fact checking as an example, in which a claim $X$ needs to be classified as whether it is supported (0) or refuted (1) with the accompanying documents $\bm{D}$.
% Inspired by prompting~\cite{brown2020language}, instead of directly inputting $X, Z$ and outputting $0/1$, we connect them with instructional prompts.
% % The input to the seq2seq model is ``A claim to be investigated is that $X$ [SEP] We have following facts: $Z_1$ $Z_2$''.
% %$P(Y|Z_1, Z_2)$ is then normalized between two outputs: ``The claim is thus supported'' or ``The claim is thus refuted''.
% For multiple-choice QA, we consider a general case where there is a varying number of choices per example, and an unknown number of the choices is correct.
% We note that determining the truth value of one answer choice may not require all sentences in the rationale; therefore, knowing the truth value of one answer choice does not have enough information to inform the entire rationale.
% For this reason, we stack all answer choices attached with their truth values as outputs to supervise the model.
% % The input to the seq2seq model is ``Question: $X$ [SEP] $Z_1$ $Z_2$''.
% % The output to be generated is ``Answer: {Choice A} {correct/wrong} [SEP] ... [SEP] Answer: {Choice N} {correct/wrong}''.
% % Each choice bracket is filled by the answer choice text.
% Finally, extractive QA can naturally be formulated as a text-to-text problem, where the input is $X$ [SEP] $Z$, and the output is $Y$.

% \subsection{Training \& Inference}
% To learn an explainable multi-hop QA system, \eba \ maximizes the likelihood function $\mathcal{L}(\cdot)$ with respect to parameters $\theta$ for all training examples:
% \begin{equation*}
%     \mathcal{L(\theta)} = \text{log} \sum_{D_1, D_2, Z_1, Z_2} P_\theta(Y, Z_1, Z_2, D_1, D_2).
% \end{equation*}
% However, when the number of documents is large or when the documents have many sentences, computing $\mathcal{L}(\theta)$ becomes intractable.
% We thus describe an approximation to this objective.
% Let $\mathcal{S}_d = \argtopk_{D_1,D_2} P_\theta(D_1, D_2)$.
% Let $z_d=(z_1, z_2)$ be a rationale from a given pair of documents $d=(d_1, d_2)$, and $\mathcal{S}_{z, d} = \argtopk_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2)$.
% Then,
% \begin{equation*}
%     \mathcal{L(\theta)} \approx \text{log} \sum_{d\in \mathcal{S}_d} \sum_{z_d\in \mathcal{S}_{z, d}} P_\theta(Y, Z_1, Z_2, D_1, D_2).
% \end{equation*}
% At test time, we choose a pair of documents by
% \begin{equation*}
%     d_1, d_2 = \argmaxB_{D_1, D_2} P_\theta(D_1, D_2).
% \end{equation*}
% Then, we choose a rationale by
% \begin{equation*}
%     z=\argmaxB_{Z_1, Z_2} P_\theta(Z_1|D_1=d_1) P_\theta(Z_2|D_2=d_2).
% \end{equation*}
% Finally, for span-based QA, we generate an answer by performing greedy search on $P(Y|Z_1,Z_2=z)$; for Boolean QA or multiple-choice QA, we normalize the answers between different choices and take $\argmaxB_{Y}P(Y|Z_1,Z_2=z)$.
